On (Omega-)Regular Model Checking

Checking infinite-state systems is frequently done by encoding infinite sets of states as regular languages. Computing such a regular representation of, say, the set of reachable states of a system requires acceleration techniques that can finitely compute the effect of an unbounded number of transitions. Among the acceleration techniques that have been proposed, one finds both specific and generic techniques. Specific techniques exploit the particular type of system being analyzed, e.g. a system manipulating queues or integers, whereas generic techniques only assume that the transition relation is represented by a finite-state transducer, which has to be iterated. In this paper, we investigate the possibility of using generic techniques in cases where only specific techniques have been exploited so far. Finding that existing generic techniques are often not applicable in cases easily handled by specific techniques, we have developed a new approach to iterating transducers. This new approach builds on earlier work, but exploits a number of new conceptual and algorithmic ideas, often induced with the help of experiments, that give it a broad scope, as well as good performances.

==> figs/conclusion.tex <==
\section{Conclusion}
\label{conclu}
Attempting to verify infinite-state systems while working exclusively
with au\-tomata-theoretic representations and algorithms can appear as
a somewhat qui\-xot\-ic endeavor. Indeed, working with domain-specific
representations will in most cases be more efficient. But, this
efficiency is gained at the price of limited applicability, sometimes
even within the chosen domain, for instance restricting oneself to
convex sets while dealing with constraints. This is to be contrasted
with the fact that the automaton-based representation used
in this article has, for instance, the unique capability of
algorithmically handling arbitrary combinations of linear constraints
involving both reals and integers. Also, a single representation
makes the handling of multiple domains direct and, for some domains
such as parametric systems, words and automata are the only available
representation.

Furthermore, the results of this article show that accelerating
sequences of automata can be done without any specific attention to
what the automata actually represent or any, a priori, restriction on
their structure. To some extent, this possibility is already partially
presented in earlier work, but making it available for infinite-word
automata is unique and very useful from the point of view of the
applications that can be handled.

Techniques for iterating sequences of automata are still in their
infancy and there is room for much further work. The set of examples
we have handled is still limited and there are many other examples to
explore and to learn from in order to improve our technique. Our
implementation has to be improved, and the procedure for checking
preciseness needs to be refined. Finally, there are a number of
possible extensions, one being to handle tree automata
\cite{ADLR05a,BHRV05}, or more general graph structures such as those of \cite{CTTV04}.



==> figs/counters.tex <==
\section{Counter automata}
\label{counters}

In this section we consider {\em counter automata}, that is a class of
automata whose transition labels are augmented with a series of
natural numbers. Those numbers can be summed to associate one or
several counter values to each word accepted by the automaton.

\begin{definition}
\label{counter-automata}
A counter automaton is an automaton $A_c=(Q,\Sigma
{\times}{\lbrack}0{\dots}d{\rbrack}^n, q_0, \delta,$\\$F)$, where $d$ and
$n$ are two integers, with $d~{\geq}~0$ and $ n > 0$.
\end{definition}

Due to their definition, counter automata can be viewed as automata on
the alphabet
$\Sigma{\times}{\lbrack}0{\dots}d{\rbrack}^n$. Consequently, the
semantic and the operations defined on automata still stand. In
addition to this, the natural numbers associated to each transition
can be used to extend the semantic as well as to define new
operations. To introduce those new concepts, it is convenient to
consider the following definition that ensures that each word is
associated with finite counter values.

\begin{definition}
A B\"uchi (weak) counter automaton $A_c=(Q,\Sigma
{\times}{\lbrack}0{\dots}d{\rbrack}^n, q_0, \delta,F)$ has the bounded
property iff for each $w_c = w(1)w(2)w(3){\dots}$ $\in$ $L(A_c)$,
there exists an index $i$ such that for each $j \ {\geq} \ i$, $w(j)$
$\in$ $(\Sigma,0^{n})$.
\end{definition}

In the rest of this article, we assume that B\"uchi (weak) counter
automata have the bounded property.

We now define two extra notions of accepted languages. They allow us
to distinguish the symbolic part of a word in $L(A_c)$ from its
numerical part. We start with $L_c(A_c)$ that links the symbolic part
of an accepted word to its counter values. Concretely, $L_c(A_c)$ is
the set of tuples $(w,v(c_1),{\dots},v(c_n))$ such that there exists a
word $w_c = (w_1,c_{11},c_{21},{\dots}c_{n1}),(w_2,$
$c_{12},c_{22},{\dots}c_{n2}),\dots$ $\in$ $L(A_c)$, where (1) for
each $i$ $\in$ $1~{\leq}~i~{\leq}~n$, $v(c_i) = \sum_{l}c_{il}$, and
(2) $w = w_1w_2\dots$; Given $w_c\in L(A_c)$, we define $P(w_c)$
to be the tuple $(w,v(c_1),{\dots},v(c_n))$, where $w$ and
$v(c_1),{\dots},v(c_n)$ are defined as above. We also define a notion
of accepted language that only considers the non-numerical part of an
accepted word, i.e. $L_\Sigma(A_c)$ $=$
${\lbrace}w=w_1w_2{\ldots}|\exists w_c\in L(A_c), w_c =
(w_1,c_{11},c_{21},{\dots}c_{n1}),(w_2,$
$c_{12},c_{22},{\dots}c_{n2}),\dots{\rbrace}$.

We now extend the operations introduce at the end of Section
\ref{transdu} to take the counters into account. Consider two counter
automata $A_{c}^1=(Q_1,\Sigma \times
{\lbrack}0{\dots}d{\rbrack}^{n_1}, q_{01},$\\$ \delta_1,F_1)$ and
$A_{c}^2=(Q_2,\Sigma \times {\lbrack}0{\dots}d{\rbrack}^{n_2},
q_{02}, \delta_2,F_2)$. The counter intersection $A_{c}^1 \cap_c
A_{c}^2$ is the counter automaton $A_{c}^{12}=(Q_1 {\times} Q_2,\Sigma
\times{\lbrack}0{\dots}d{\rbrack}^{n_1+n_2}, (q_{01},q_{02}),
\delta_{12},F_1 \times F_2)$, where
\begin{multline*}
\delta_{12}((q_1,q_2),(b,c_{1i}{\dots}c_{(n_1 + n_2)i})=\{(q'_1,q'_2)\mid (q'_1 \in \delta_1(q_{1},(b,c_{1i},{\dots},c_{n_1i})))\ \\ \mbox{and}\ q'_2 \in
\delta_2(q_2,(b,c_{(n_1+1)i},{\dots},c_{(n_1+n_2)i}))\}.
\end{multline*}

Consier two counter transducers
$T_{c}^{1}=(Q_1,\Sigma \times {\lbrack}0{\dots}d{\rbrack}^{n_1},
q_{01}, \delta_1,F_1)$ and $T_{c}^{2}=(Q_2,\Sigma \times
{\lbrack}0{\dots}d{\rbrack}^{n_2}, q_{02}, \delta_2,F_2)$. The counter
composition $T_{c}^{1}{\circ_{c}}T_{c}^{2}$ is the transducer
$T_{c}^{12}=(Q_1 {\times} Q_2,\Sigma \times \Sigma
\times{\lbrack}0{\dots}d{\rbrack}^{n_1+n_2}, (q_{01},q_{02}),
\delta_{12},$ $F_1 \times F_2)$, where
\begin{multline*}
\delta_{12}((q_1,q_2),((a,b),c_{1i}{\dots}c_{(n_1 + n_2)i})=\{(q'_1,q'_2)\mid (\exists c \in \Sigma) \\ (q'_1 \in \delta_1(q_{1},((a,c),c_{1i},{\dots},c_{n_1i})))\ \mbox{and}\ q'_2 \in
\delta_2(q_2,((c,b),c_{(n_1+1)i},{\dots},c_{(n_1+n_2)i}))\}.
\end{multline*}

Given a transducer
$T=(Q_3,\Sigma,q_{03},\delta_3,F_3)$, the composition
$T(A_{c}^1)_c$ is a counter automaton $A_{c}^{13}=(Q_1 {\times}
Q_3,\Sigma
\times{\lbrack}0{\dots}d{\rbrack}^{n_1},(q_{01},q_{03}),$ $
\delta_{13},F_1 \times F_3)$, where
\begin{multline*}
\delta_{13}((q_1,q_3),(b,c_{1i}{\dots}c_{n_1i})=\{(q'_1,q'_3)\mid (q'_3 \in \delta_3(q_3,(a,b))\  
\\ \mbox{and}\ q'_1 \in
\delta_1(q_1,(a,c_{1i},{\dots},c_{n_1i}))\}.
\end{multline*}

Finally, it is possible to define a projection operation that selects
words if they satisfy a constraint on their counter values. Let
$a_1,{\dots},a_x,i$ $\in$ ${\lbrack}1{\dots}n{\rbrack}$ be different
indexes. We define $\pi_{c_i > c_{a},{\dots},c_{ax}}(A_{c})$ to be a
counter automaton $A'$ whose language is the set of words $w_c' =
(w_1,c_{i1})(w_2,c_{i2}){\dots}$ such that there exists $w_c =
(w_1,c_{11},c_{21},{\dots}c_{n1}),(w_2,c_{12},c_{22},{\dots}c_{n2}),\dots$
$\in$ $L(A_{c})$, where $P(w_c) = (w,v(c_1),{\dots},$\\$v(c_n))$ and, if
$v(c_i) > 0$, then for each $(i < j~{\leq}~x)$, $v(c_{aj}) < v(c_i)$.






==> figs/counting.tex <==
\section{Counting the Steps}
\label{count-step}

In this section, we extend the alphabet of the automaton  $A_{e_*}$ by adding positiv numbers to it transitions.\\
\newline
I need one of you to explain in english the utility of those numbers.\\

Consider a transition labeled by a symbol $a$ that goes from a state
$x$ of $Q_{I_0}$ to a state $y$ of $Q_{I_3}$. By applying the
extrapolation principle describe in the previous section, we will add
a transition labeled by $a$ between the state $x$ of $Q_{I_0}$ and the
state $y$ of $Q_{I_2}$. This transition simulate the existence of one
more increment. It can thus be labeled with a counter value of $1$. We
can generalize this principle to each added transition. This situation
is illustrated at Figure \ref{extra-algo2}.

\begin{figure}
\begin{center}
\input{figs/figs/extrapolation2.pstex_t}
\end{center}
\caption{find a title}
\label{extra-algo2}
\end{figure}

We now introduce extended automata.

\begin{definition}
An extended automaton $A_{c}=(Q,
\Sigma{\times}{\lbrack}0{\dots}c{\rbrack}, q_0, \delta, F)$ is an
automaton such that each of its transitions owns a counter value,
which is a positive (or zero) integer that is less than a constant
$c$.
\end{definition}

plus petit que i.
\begin{definition}
We denote by $A_{c=i}$ the counter automaton $A_{c}$ that accepts only
words when the sum of the counter values is $i$.
\end{definition}

\begin{definition}
The non-counter language accepted by a counter automaton $A_{c}=(Q,
\Sigma{\times}{\lbrack}0{\dots}c{\rbrack}, q_0, \delta, F)$ is the set
of pairs $(w,i)$ such that:
\begin{itemize}
\item
the word $w \in L(A_{c}$;
\item
the sum of the counter values of each transitions followed by the run
of $w$ is equal(resp ${\leq}$) $i$.
\end{itemize} 
\end{definition}

\begin{definition}
We denote by $A_{c=i}$ the counter automaton $A_{c}$ that accepts only
words when the sum of the counter values is $i$.
\end{definition}

\begin{definition}
Let $A_{c}=(Q,{\Sigma},{\delta},I,F)$ be a counter
automaton, we denote by $L_{({\Sigma})}(A_{c})$ the
set of words $w$ such that there exists a $i{\geq}0$ and $(w,i)$ is
accepted by $A_{c=i}$.
\end{definition}
\begin{definition}
A counter automaton $A_{c}$ is structurally equivalent to an automaton
$A$ if $L_{\Sigma}(A_{c})=L(A)$
\end{definition}

We now formalize the construction of an extended automaton structurally
equivalent to $A^{e_*}$ and such that the transitions own counter
values that count the number of increments they simulate.

\begin{algo}
\label{closure_algo_2}
For each state $q \in Q_{I_0}$ and $a \in \Sigma$,
\begin{enumerate}
\item
If $\delta(q,a)$ is a state $q'$ that belongs an increment
$Q_{I_{j}}$, $1\leq j \leq k -1$, then
\item
add transitions from $q$ and labeled by $a$ to the state corresponding
to $q'$ (by the increment isomorphism) in each of the increments
$Q_{I_{\ell}}^{s_{i+k}}$ with $0\leq \ell < j$ and add the counter
value $j-l$ to this transition,
\item 
set the counter value to zero for all the other transitions.
\end{enumerate}
\end{algo}

All these definitions can be directly generalized to the case of a
multi-counters automaton, i.e. an automaton which transitions own more
than one counter value.

We have the following theorem.

\begin{theorem}
Consider an automaton $A^{e_0}$ such that its state set $Q$ can be
decomposed into a head part $Q_H$, a series of $k$ increments
$Q_{I_0}, \ldots, Q_{I_{k-1}}$, and a tail end part $Q_{T_f}$. Let
$A_x$ be the automaton obtained after applying Algorithm
\ref{closure_algo_1} to $A^{e_0}$ and $A_y$ be the automaton obtained
after applying Algorithm \ref{closure_algo_2} to $A^{e_0}$. We have
that $A_y$ is structurally equivalent to $A_x$.
\end{theorem}

\begin{proof}
It suffices to remark that the rules of Algorithm \ref{closure_algo_1}
are identical to those of Algorithm \ref{closure_algo_2} if we except
manipulations on counters.
\end{proof}

In this section, we have presented algorithms that are able to
extrapolate a finite sampled sequence of automata. The extrapolation
is based on properties of the finite sequence. Because there are no
guarantee that these properties remains true for the infinite
sequence, we must prove that our extrapolation is a good extrapolation
i.e. we must prove that it really represent the infinite sequence. For
doing this we have developed two criteria, which are presented in the
next chapter.


==> figs/experiments.tex <==
\section{Experiments}
\label{expe}

The techniques proposed in this article have been tested on several case
studies, using an implementation that relies on the LASH
package~\cite{LASH} for handling automata. This section describe some
of the experiments that have been conducted with the tool.

We first used the implementation to compute the exact reachable set of
states of several parametric systems proposed in
\cite{Tou01,Tou03}. Our experiments included a token ring, a Bakery
algorithm, a Szymanski algorithm, a Burns algorithm, and a Dijkstra
algorithm. In all the cases we considered, the sampling sequence was
linear. In table \ref{tbl-parametric}, we give the number of states of
the minimal and deterministic form of the automaton representing the
initial set of configurations, of the transducer representing the
transition relation, and of the computed closure. Note that the
computation of $T^*(A_{\phi_I})$ was done without any manual
intervention and any computation of transitive closure of
actions. This is in contrast with \cite{BJNT00,Tou01,Tou03} in where
the computation was done by first computing the transitive closure for
each individual action, and then applying a classical forward
reachability algorithm using these results. However, when considering
parametric systems, such an approach requires manual intervention: to
make the reachability analysis terminate, it is often necessary to
combine actions in a certain order, or even to accelerate combinations
of individual actions.  On the bad side, we have been able to
compute the transitive closure of individual actions of the protocols,
but not of the entire transition relation (\cite{AJNdo03}).

\begin{table}
\begin{center}
\begin{tabular}{|c|r|r|r|r|}
\hline
Relation&$~|A_{\phi_I}|~$&$~|T_0|~$&$~|A_{\phi_I}^*$\\
\hline
Token Ring & 2 & 7 & 2\\
Bakery & 1 & 6 & 3 \\
Szymanski & 1 & 14 & 7 \\
Burns & 1 & 4 & 2 \\
Dijkstra & 2 & 9 & 2 \\
\hline
\end{tabular}
\end{center}
\vspace{0.75em}
\caption{Results for parametric Systems.}
\label{tbl-parametric}
\end{table}

A second series of test cases consisted of handling systems that
manipulate unbounded integer variables. Positive integers were encoded
in binary with an arbitrary number of leading $0$'s allowed, and
negative numbers were represented using $2$'s complement allowing for
an arbitrary number of leading $1$'s, following the encoding presented
in \cite{WB00}. We first computed an upper-approximation of the
transitive closure of several transducers representing arithmetic
relations. In all the cases we considered, the sampling sequence
consists of the powers of $2$. In Table~\ref{tbl-ex1} we give the
number of states of some transducers that were iterated, of their
closure, and of the largest power of the transducer that was
constructed. Using the same encoding we also computed the reachable
set of states of the {\em lift} and {\em producer-consummers}
algorithms proposed in \cite{BFLS05,BLP06}.


\begin{table}
\begin{center}
\begin{tabular}{|c|r|r|r|}\hline
Relation&$~|T_0|~$&$~|T_0^*|~$&~Max $|T_0^i|~$\\
\hline
$(x,x+1)$&3&3&9\\ 
$(x,x+73)$&14&75&637\\
$(x,x+1777)$&23&14481&1779\\
$((x,y),(y+17,x-19))\cap\, \nats^2 \times \nats^2$&120&935&8393\\
$(((x,y),(x+2,y-1))\,\cup\,
((x,y),(x-1,y+2)))$&&&\\
$\cap\, \nats^2 \times \nats^2$
&20&71&1084\\
$((x,y),(x+2,y-1))\,\cup\,
((x,y),(x-1,y+2))$&&&\\
$\,\cup\,
((x,y),(x+1,y+1)))\, \cap\, \nats^2 \times \nats^2$
&22&33&492\\
$((w,x,y,z),(w+6,x+2,y+3,z+5))$&146&585&3793\\ 
\hline
\end{tabular}
\end{center}
\vspace{0.75em}
\caption{Computation of the reflexive closure of relations of systems
that manipulate integer variables.}
\label{tbl-ex1}
\end{table}

We then considered systems with real variables. In this case, both the
transition relation and the set of configurations were represented by
{\em Real Vector Automata\/}~\cite{BBR97,BJW01}, i.e., B\"uchi
automata operating over the binary encoding of numbers.

\begin{figure}
\centerline{\input{figs/gas-burner.pstex_t}}
\caption{Hybrid automaton modeling the leaking gas burner.}
\label{hyb-burner}
\end{figure}

One of our case studies consisted of computing the closure of the
transition relation of the {\em leaking gas burner\/} described
in~\cite{ACHH95}. This system consists in a gas burner that leaks
during periods of less than one time unit (t.u.), these periods being
separated by at least $30$ t.u. A linear hybrid automaton modeling the
leaking gas burner is given in Figure \ref{hyb-burner}. The states $L$
and ${\neg}L$ correspond respectively to the leaking and non-leaking
situations, $x$ measures the leaking periods and the interval between
them, $y$ is absolute time, and $z$ keeps track of the cumulated
leaking duration. With our implementation, we were able to compute a
superset of its reachable set of configurations. We then compared this
set with the one produced by the technique described in~\cite{BHJ03}
(which is specific to linear hybrid automata), from which it turned
out that our computed set was actually exact. For this case study, the
minimal and deterministic form of the transition relation is a
transducer with $2406$ states, and the representation of the
reachability set has $524$ states. The largest automaton considered by
the increment detection procedure had $1892$ states.  Our
implementation was also applied to other case studies such as a
simplified model of the root contention protocol \cite{SS01} described
in \cite{Boi04}. We also considered several relations coming from
communication protocols. In this last case, we used the encoding given
in \cite{JN00}.



==> figs/extra-count.tex <==
\subsection{Adding Counters}
\label{count}

In this section, we extend Algorithms \ref{closure_algo_1} and
\ref{closure_algo_3}, by adding a counter increments to the label of each 
transition of the automaton $A^{e_*}$. This is done to count the
number of increments simulated when following a transition. Such
constructions will be intensively used in Section
\ref{safe-precis}, when developing criteria to check the exactness of
an extrapolation. Given $d$, the communication diameter of $A^{e_0}$,
we build a counter automaton $A_c^{e_*}$ on the alphabet $\Sigma
\times \lbrack 0 {\dots} d \rbrack$, such that (1) for each $(w,i)$
$\in$ $L_{c}(A^{e_*}_c)$, $w$ $\in$ $L(A^{e_i})$, and (2) for each $w$
$\in$ $L(A^{e_i})$, there exists $(w,j~{\leq}~i)$ $\in$
$L_c(A^{e_*}_c)$. This can be done with a small extension in
Algorithms \ref{closure_algo_1} and \ref{closure_algo_2}.

We start with the case of finite words. 

\begin{algo}
\label{closure_algo_2}
Consider the finite word automaton $A^{e_0} = (Q^{e_0},
\Sigma, q_0^{e_0},$\\$\delta^{e_0}, F^{e_0})$. We build a finite-word
counter automaton $A^{e_*}_c = (Q^{e_*}, \Sigma {\times}
{\lbrack}0{\dots}d{\rbrack}, q_0^{e_*},$\\$\delta^{e_*}, F^{e_*})$, where
$Q^{e_*} = Q^{e_0}$, $q_0^{e_*} = q_0^{e_0}$, $F^{e_*} = F^{e_0}$. Each state
$q^{e_*}$ of $A^{e_*}$ is associated to exactly one state $q^{e_0}$ by
a relation $\equiv~{\subseteq}~Q^{e_0} \times Q^{e_*}$. Moreover
$Q^{e_*}$ can be decomposed into $Q_H^{e_0}~{\equiv}~Q_H^{e_*}$, a
series of $k$ increments $Q_{I_0}^{e_0}~{\equiv}~Q_{I_0}^{e_*},
\ldots, Q_{I_{k-1}}^{e_0}~{\equiv}~Q_{I_{k-1}}^{e_*}$, and a final
tail $Q_{T_f}^{e_0}~{\equiv}~Q_{T_f}^{e_*}$. The transition relation
$\delta^{e_*}$ is built in the following way. For each
transition $(q_x^{e_i},a,q_y^{e_i})$ in $A^{e_0}$, there is a
transition $(q^{e_*}_x,(a,0),q^{e_y^{e_*}})$ in $A^{e_*}_c$, ,with
$q_x^{e_0} \equiv q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.  For
each state $q \in Q_{H}~{\cup}~Q_{I_0}$ and for every $a \in \Sigma$,
\begin{quote}
If $\delta^{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}$, $1\leq j \leq k -1$, then for each increment
$Q_{I_{\ell}}^{e_*}$ with $0\leq \ell < j$, there is a transition
$(q_x^{e_*},(a,j-l),(q_y^{e_*})')$ in $A^{e_*}_c$, where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, and $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.
\end{quote}
\end{algo}

\begin{figure}
\begin{center}
\input{figs/figs/extra2.pstex_t}
\end{center}
\caption{Illustration of the extrapolation algorithm for
finite-word automata with the addition of counters.
\label{extra-algo3}
}
\end{figure}

\begin{example}
Figure \ref{extra-algo3} sketchs the application of Algorithm
\ref{closure_algo_2} on the example given in Figure \ref{extra-algo2}.
\end{example}

We can generalize the construction to the $\omega$-words case, by
following the same idea.

\begin{algo}
\label{closure_algo_4}
Consider the deterministic B\"uchi weak automaton $A^{i+k} = A^{e_0} =
(Q^{e_0}, \Sigma, q_0^{e_0}, \delta^{e_0}, F^{e_0})$. We build a
B\"uchi weak counter automaton $A^{e_*}_c = (Q^{e_*}, \Sigma
{\times}{\lbrack}0{\dots}d{\rbrack}, q_0^{e_*}, \delta^{e_*},
F^{e_*})$, where $Q^{e_*} = Q^{e_0}~\cup~Q_{I_{0}COPY}$, $q_0^{e_*} =
q_0^{e_0}$, $|Q_{I_{0}COPY}|=|Q_{I_0}^{e_0}|$ , and $F^{e_*} =
F^{e_0}$. Each state $q^{e_0}$ of $A^{e_0}$ is associated to exactly
one state $q^{e_*}$ of $A^{e_*}_c$ by a relation $\equiv_1~{\subseteq}~Q^{e_0} \times (Q^{e_*}-Q_{I_{0}COPY})$. ²qMoreover
$Q^{e_*}-Q_{I_{0}COPY}$ can be decomposed into $Q_H^{e_0}~{\equiv_1}~Q_H^{e_*}$, a series of $k$ increments $Q_{I_0}^{e_0}~{\equiv_1}~Q_{I_0}^{e_*}, \ldots, Q_{I_{k-1}}^{e_0}~{\equiv_1}~Q_{I_{k-1}}^{e_*}$, and a final tail $Q_{T_f}^{e_0}~{\equiv_1}~Q_{T_f}^{e_*}$.  The set $Q_{I_{0}COPY}$ is used to create a copy of
$Q_{I_{0}}^{e_0}$.  Each state of $Q_{I_{0}COPY}$ is associated to a
corresponding state in $Q_{I_{0}}^{e_*}$ by a relation $\equiv_2
{\subseteq}Q_{I_{0}}^{e_*}{\times}Q_{I_{0}COPY}$. The set of
transition is built in the following way. For each transition
$(q_x^{e_0},a,q_y^{e_0})$ in $A^{e_0}$, there exists a transition
$(q_x^{e_*},(a,0),q_y^{e_*})$ in $A^{e_*}$ with $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.  For each transition
$(q_x^{I_0},a,q_y^{I_0})$ in $A^{e_*}$ with $q_x^{I_0},q_y^{I_0}$
$\in$ $Q_{I_0}^{e_*}$ there exists a transition
$(q_x^{I_{0}COPY},(a,0),q_y^{I_{0}COPY})$ where $q_x^{I_{0}COPY}$ and
$q_y^{I_{0}COPY}$ $\in$ $Q_{I_{0}COPY}$ and $q_x^{I_0} \equiv_2
q_x^{I_{0}COPY}$ and $q_y^{I_0} \equiv_2 q_y^{I_{0}COPY}$.  For each
transition $(q_x^{I_0},a,q_y^{e_*})$ in $A^{e_*}$ with $q_x^{I_0}$
$\in$ $Q_{I_0}^{e_*}$ and $q_y^{e_*}$ $\not\in$ $Q_{I_0}^{e_*}$, there
exists a transition $(q_x^{I_{0}COPY},(a,0),q_y^{e_*})$ where
$q_x^{I_{0}COPY}$ $\in$ $Q_{I_{0}COPY}$ and $q_x^{e_*}
\equiv_2q_x^{I_{0}COPY} $. For each state $q \in Q_{H}^{e_0} \ {\cup}
\ Q_{I_0}^{e_0}$ and for every $a \in \Sigma$,
\begin{enumerate}
\item
 if $\delta_{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}^{e_0}$, $1\leq j \leq k -1$, then for each
increment $Q_{I_{\ell}}^{e_*}$ with $0 < \ell < j$, there is a
transition $(q_x^{e_*},(a,j-l),(q_y^{e_*})')$ in $A^{e_*}_c$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, with $q_x^{e_0}
\equiv_1 q_x^{e_*}$ and $q_y^{e_0} \equiv_1 q_y^{e_*}$. There is also
a transition $(q_x^{e_*},(a,j),q_y^{I_{0}COPY})$, where
$q_y^{I_{0}COPY}$ is the state corresponding to $q_y^{e_*}$ in
$Q_{I_{0}COPY}$ by the increment isomorphism.
\item
 if $q$ $\in$ $Q^{e_0}_{I_0}$ then let $q^{I_{0}COPY}$ be the state
corresponding to $q$ in $Q_{I_{0}COPY}$ (i.e. $(q,q^{I_{O}COPY}$) $\in$
$\equiv_2 {\circ} \equiv_1$ ). For each increment $Q_{I_{\ell}}^{e_*}$
with $1~{\leq}~l < j$, there is a transition
$(q^{I_{0}COPY},(a,j-l),(q_y^{e_*})')$ in $A^{e_*}_c$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$. There is also a
transition $(q^{I_{0}COPY},(a,j),q_y^{I_{0}COPY})$, where
$q_y^{I_{0}COPY}$ is the state corresponding to $q_y^{e_*}$ in
$Q_{I_{0}COPY}$.
\end{enumerate}
\end{algo}

\begin{figure}
\begin{center}
\input{figs/example2.pstex_t}
\end{center}
\caption{Application of Algorithm \ref{closure_algo_4} to the automaton
of Figure \ref{example-auto}}.
\label{example-auto22}
\end{figure}
\begin{example}
Figure \ref{example-auto22} shows the result of applying Algorithm
\ref{closure_algo_4} to the automaton $A^{3}$ of Figure
\ref{extra-algo2}.
\end{example}

Note that in both cases, $A^{e_*}_c$ is, by construction,
deterministic. Moreover, in the $\omega$-word case, each run on a word
$w_c\in L(A^{e_*}_c)$ (resp. $w\in L(A^{e_i{\geq}0})$) has the
following form: $q_1{\dots}q_n(sc)^{\omega}$, where $sc$ is a strongly
connected component of $A^{e_*}_c$ (resp. $A^{e_i{\geq}0}$) such that
$sc~{\subseteq}~F^{e_*}$ (resp. $sc~{\subseteq}~F^{e_i}$).

\begin{theorem}
\label{accepting-SC}
In the $\omega$-word case, the automaton $A^{e_*}_c$ has the bounded
property.
\end{theorem}

\begin{proof}
Let $SC^{e_*}$ be the set of strongly connected components of
$A^{e_*}_c$. For each $sc$ $\in$ $SC^{e_*}$, if $sc \cap F^{e_*} \not=
{\emptyset}$, then $sc~\subseteq~Q^{e_0}$, and the result holds since
the transitions of those strongly connected components are augmented
with a counter increment whose value is $0$.
\end{proof}

We have the following correctness results.

\begin{theorem}
\label{th-algo-count1}
For all $w_c$ on the alphabet $\Sigma {\times}
{\lbrack}0{\dots}d{\rbrack}$, with $P(w_c) = (w,i)$, $w_c \in
L(A^{e_*}_c) \Rightarrow w
\in L(A^{e_{i}})$.
\end{theorem}

\begin{proof}
See Appendix \ref{app1}.
\end{proof}

\begin{theorem}
\label{th-algo-count2}
For all $w$ $\in$ $L(A^{e_i})$, there exists $w_c$ $\in$
$L(A^{e_*}_c)$ with $P(w_c) = (w,j)$, and $j~{\leq}~i$.
\end{theorem}

\begin{proof}
See Appendix \ref{app1}.
\end{proof}

Finally, we have the following corollary.
 
\begin{corollary}
\label{corollary-count}
$L_{\Sigma}(A^{e_*}_c) = L(A^{e_*})$.
\end{corollary}

\begin{proof}
Obvious.
\end{proof}

Note that, Lemma \ref{corollary-count} gives a formal proof of
correctness of Algorithms \ref{closure_algo_1}, and
\ref{closure_algo_3}. 





==> figs/extra-deux.tex <==
\section{An Extrapolation Step for Sequence of Automata}
\label{extrap-1}

In this section, we consider an incrementally growing sequence
$A^{i}$, $A^{i + 1}$, \ldots, $A^{i + k}$ of finite-word
(resp. B\"uchi weak) automata, which are assumed to be deterministic
and minimal. For each $j$ $\in$ $0~{\leq}~j~{\leq}~k$, $A^{i+j} =
(Q^{i+j}, \Sigma, q_0^{i+j}, \delta^{i+j}, F^{i+j})$.

Consider the automaton $A^{i+k}$ of the sequence to which the
extrapolation step described at the end of the last section can be
applied. This automaton is for notation reasons renamed into
$A^{e_0}$. Following definitions \ref{def-incr-larger1}, the state set
$Q^{e_0}$ of $A^{e_0}$ can be decomposed into a head part $Q_H^{e_0}$,
a series of $k$ increments $Q_{I_0}^{e_0}, \ldots, Q_{I_{k-1}}^{e_0}$,
and a tail end part $Q_{T_f}^{e_0}$. Repeatedly applying the
extrapolation step described at the end of the previous section
generates an infinite sequence of finite-word (resp. B\"uchi weak)
automata
$A^{i},A^{i+1},{\dots},A^{i+k-1},A^{e_0}A^{e_1},A^{e_2}{\dots}$ that
grows incrementally, and such that (1) for each $j$ $\in$
$0~{\leq}~j~{\leq}~k$, $A^{e_j} = (Q^{e_j}, \Sigma, q_0^{e_j},
\delta^{e_j}, F^{e_j})$, (2) $\forall i > 0$, $Q_H^{e_i}$ is
communication stable with $Q_H^{e_0}$, and (3) $\forall i > 0$,
$Q_{I_0}^{e_i}$ is communication equivalent to $Q_{I_0}^{e_0}$.

Our goal is to build a single finite-word (resp. B\"uchi weak)
automaton that captures the behavior of the automata in this sequence,
i.e. $A^{e_*}={\bigcup}_{i{\geq}0}A^{e_i}$.

We develop separated solutions for finite-word and B\"uchi weak
automata.

{\em Remark.} If one dissects the previous definitions, one easily
note that there exists an isomorphism between the graphs induced by
the states of both the head parts of the $A^{e_i}$ and the head part
of $A^{e_*}$. The same apply for increments that are detected in those
structures. For facility reasons, we will assume the existence of
those isomorphism relations, but we wont give a formal definition to
simplify notations.

\subsection{The Finite word Case}
\label{extra}

We aim at computing a finite representation of $A^{e_*}$ from a
sequence of finite-word automata. The idea is to build $A^{e_*}$ from
$A^{e_0}$ by adding new transitions that simulate the existence of
additional increments.

Consider a transition labeled by a symbol $a$ that goes from a state
$x$ of $Q_{I_0}^{e_0}$ to a state $x'$ of $Q_{I_3}^{e_0}$ and a
transition labeled by $b$ that goes from a state $y$ of $Q_H^{e_0}$ to
a state $y'$ of $Q_{I_2}^{e_0}$. Consider now $A^{e_1}$, this
finite-word automaton is incrementally larger than $A^{e_0}$. Since,
the increment $Q_{I_0}^{e_1}$ added between $A^{e_0}$ and $A^{e_1}$ is
also communication equivalent to $Q_{I_0}^{e_0}$ there must exists a
transition labeled by a symbol $a$ from the state of $Q_{I_0}^{e_1}$
that is isomorphic to $x$ to the state that is isomorphic to $x'$ in
$Q_{I_2}^{e_1}$. We do not want to add the new increment, but we can
simulate its existence by using $Q_{I_0}^{e_0}$ and by adding a
transition labeled by a symbol $a$ from the state $x$ of
$Q_{I_0}^{e_0}$ to the state isomorphic to $x'$ in
$Q_{I_2}^{e_0}$. The same idea can be repeated if we add two or three
increments. Simulating more than three increments can be done by using
states of $Q_{I_0}^{e_0}$. Due to the communication equivalence
property, a transition labeled by $b$ must also be added between the
state $y$ of $Q_H^{e_0}$ and the state that is isomorphic to $y'$ in
$Q_{I_1}^{e_0}$. The situation is illustrated in Figure
\ref{extra-algo1}, where the dashed transitions are the transitions
added during the extrapolation process.\\

\begin{figure}
\begin{center}
\input{figs/figs/extra1.pstex_t}
\end{center}
\caption{Illustration of the extrapolation algorithm for
finite-word automata.
\label{extra-algo1}
}
\end{figure}

Formally, the finite-word automaton $A^{e_*}$ can be built from $A^{e_0}$ by
adding transition with the following algorithm.

%% In the algorithm, I didn't know if I was supposed to also
%% give a name to the isomorphic relations between the increments.
%% Axel.

\begin{algo}
\label{closure_algo_1}
Consider the finite word automaton $A^{i+k} = A^{e_0} = (Q^{e_0},
\Sigma, q_0^{e_0},$\\$\delta^{e_0}, F^{e_0})$. We build a finite word
automaton $\widehat{A^{e_*}} = (Q^{e_*}, \Sigma, q_0^{e_*},
\delta^{e_*}, F^{e_*})$, where $Q^{e_*} = Q^{e_0}$, $q_0^{e_*} =
q_0^{e_0}$, and $F^{e_*} = F^{e_0}$. Each state $q^{e_*}$ of
$\widehat{A^{e_*}}$ is associated to exactly one state $q^{e_0}$ of
$A^{e_0}$ by a relation $\equiv~{\subseteq}~Q^{e_0} \times
Q^{e_*}$. Moreover $Q^{e_*}$ can be decomposed into
$Q_H^{e_0}~{\equiv}~Q_H^{e_*}$, a series of $k$ increments
$Q_{I_0}^{e_0}~{\equiv}~Q_{I_0}^{e_*}, \ldots,
Q_{I_{k-1}}^{e_0}~{\equiv}~Q_{I_{k-1}}^{e_*}$, and a final tail part
$Q_{T_f}^{e_0}~{\equiv}~Q_{T_f}^{e_*}$. The transition relation
$\delta^{e_*}$ is built in the following way. For each transition
$(q_x^{e_0},a,q_y^{e_0})$ in $A^{e_0}$, there exists a transition
$(q_x^{e_*},a,q_y^{e_*})$ in $A^{e_*}$ with $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$. For each state $q \in
Q_{H}^{e_0} \ {\cup} \ Q_{I_0}^{e_0}$ and for every $a \in \Sigma$,
\begin{quote}
If $\delta^{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}^{e_0}$, $1\leq j \leq k -1$, then for each
increment $Q_{I_{\ell}}^{e_*}$ with $0\leq \ell < j$, there is a
transition $(q_x^{e_*},a,(q_y^{e_*})')$ in $\widehat{A^{e_*}}$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, and $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.
\end{quote}
\end{algo}

The added transitions, which include loops (transitions to $Q_{I_0}$
itself) allow $\widehat{A^{e_*}}$ to simulate the computations of any
of the $A^{e_i}$, $i\geq 0$. Conversely, it is fairly easy to see all
computations generated using the added transitions correspond to a
computation of some $A^{e_i}$. A formal proof of the correctness of
Algorithm \ref{closure_algo_1} will be given at the end of this
section, when proving a more general result.

Let $d$ be the maximal distance of communication of $A^{e_0}$, we now
build a finite-word counter automaton $A_c^{e_*}$ on the alphabet
$\Sigma \times \lbrack 0 {\dots} d \rbrack$ such that (1)
$L_{\Sigma}(A^{e_*}_c) = L(A^{e_*})$, (2) for each $(w,i)$ $\in$
$L_{c}(A^{e_*}_c)$ $w$ $\in$ $L(A^{e_i})$, (3) for each $w$ $\in$
$L(A^{e_i})$, there exists $(w,j~{\leq}~i)$ $\in$ $L_c(A^{e_*}_c)$
. To do this, one can label the transitions that are added in algorithm
\ref{closure_algo_1} with an integer that represents the
number of increments they simulate. Figure
\ref{extra-algo2} shows the result of applying this rule on the
example given in Figure \ref{extra-algo1}.

\begin{figure}
\begin{center}
\input{figs/figs/extra2.pstex_t}
\end{center}
\caption{Illustration of the extrapolation algorithm for
finite-word automata with the addition of counters.
\label{extra-algo2}
}
\end{figure}

\begin{algo}
\label{closure_algo_2}
Consider the finite word automaton $A^{i+k} = A^{e_0} = (Q^{e_0},
\Sigma, q_0^{e_0},$\\$\delta^{e_0}, F^{e_0})$. We build a finite-word
counter automaton $A^{e_*}_c = (Q^{e_*}, \Sigma {\times}
{\lbrack}0{\dots}d{\rbrack}, q_0^{e_*},$\\$\delta^{e_*}, F^{e_*})$, where
$Q^{e_*} = Q^{e_0}$, $q_0^{e_*} = q_0^{e_0}$, $F^{e_*} = F^{e_0}$, and
$d$ is the maximal distance of communication of $A^{i+k}$. Each state
$q^{e_*}$ of $A^{e_*}$ is associated to exactly one state $q^{e_0}$ by
a relation $\equiv~{\subseteq}~Q^{e_0} \times Q^{e_*}$. Moreover
$Q^{e_*}$ can be decomposed into $Q_H^{e_0}~{\equiv}~Q_H^{e_*}$, a
series of $k$ increments $Q_{I_0}^{e_0}~{\equiv}~Q_{I_0}^{e_*},
\ldots, Q_{I_{k-1}}^{e_0}~{\equiv}~Q_{I_{k-1}}^{e_*}$, and a final
tail $Q_{T_f}^{e_0}~{\equiv}~Q_{T_f}^{e_*}$. The transition relation
$\delta^{e_*}$ is built in the following way. For each
transition $(q_x^{e_i},a,q_y^{e_i})$ in $A^{e_0}$, there is a
transition $(q^{e_*}_x,(a,0),q^{e_y^{e_*}})$ in $A^{e_*}_c$, ,with
$q_x^{e_0} \equiv q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.  For
each state $q \in Q_{H}~{\cup}~Q_{I_0}$ and for every $a \in \Sigma$,
\begin{quote}
If $\delta^{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}$, $1\leq j \leq k -1$, then for each increment
$Q_{I_{\ell}}^{e_*}$ with $0\leq \ell < j$, there is a transition
$(q_x^{e_*},(a,j-l),(q_y^{e_*})')$ in $A^{e_*}_c$, where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, and $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.
\end{quote}
\end{algo}

Note that $A^{e_*}_c$ is deterministic by construction. Moreover
$L_{\Sigma}(A^{e_*}_c) = L(\widehat{A^{e_*}})$. 


\begin{theorem}
\label{th-algo-count}
Let $A^{e_*}_c$ be the finite-word automaton obtained by applying
algorithm \ref{closure_algo_4} to $A^{e_0}$. We have that $\forall
w_c$ $\in$ $(\Sigma {\times} {\lbrack}0{\dots}d{\rbrack})^*$ such that
$P(w_c) = (w,i)$, $w_c \in L(A^{e_*}_c) \Rightarrow w \in
L(A^{e_{i}})$. Moreover, $\forall$ $w$ $\in$ $\Sigma^*$ such that $w$
$\in$ $L(A^{e_i})$, there exists $w_c$ $\in$ $L(A^{e_*}_c)$ such that
$P(w_c) = (w,j~{\leq}~i)$.
\end{theorem}


\begin{proof} 
By simplification, we suppose that $|Q_H^{e_*}|>0$. We prove the two
statements of the theorem.
\begin{enumerate}
\item

We show that for each $w_c = (w(1),c_1)(w(2),c_2){\dots}(w(n),c_n)$
$\in$ $L(A^{e_*}_c)$ with $P(w_c) = (w,i)$, there exists $w$ $\in$
$L(A^{e_i})$. The result is direct if $i = 0$. We now suppose
$i>0$. Consider the unique accepting run $\pi^{e_*} =
q_0^{e_*}q_1^{e_*}q_2^{e_*}{\dots}q_n^{e_*}$ on the word $w_c$ in
$A^{e_*}_c$. We show that there exists an accepting run $\pi^{e_i} =
q_0^{e_i}q_1^{e_i}q_2^{e_i}{\dots}q_n^{e_i}$ on the word $w$ in
$A^{e_i}$. This is done by associating a state of $A^{e_i}$ to each
state of $\pi^{e_*}$.

let $q_0^{e_*}q_1^{e_*}q_2^{e_*}{\dots}q_u^{e_*}$ be the part of
$\pi^{e_*}$ that stays in $Q_H^{e_*}$. Since $Q_H^{e_*}$ and
$Q_H^{e_i}$ are isomorphic, the corresponding states in $A^{e_i}$ are
$q_0^{e_i},q_1^{e_i},q_2^{e_i},{\dots},q_u^{e_i}$, where $q_j^{e_i}\in
Q_H^{e_i}$ and $q_j^{e_i}$ is isomorph to $q_j^{e_*}$,
$\forall{j}$ $\in$ ${\lbrack}0{\dots}u{\rbrack}$,

If $ q^{e_*}_{u+1} = \delta(q_u^{e_*},(w(u+1),c_{u+1}=i))$ and
$q^{e_*}_{u+1}$ $\in$ $Q_{I_{j{\geq}1}}^{e_*}$ then, since $A^{e_0}$
and $A^{e_i}$ are communication stable, there exists $q^{e_i}_{u+1}\in
Q_{I_{j+i}}^{e_i}$ such that $q^{e_i}_{u+1} =
\delta(q_u^{e_i},w(u+1))$ and $q^{e_i}_{u+1}$ is isomorphic to
$q^{e_*}_{u+1}$. By definition there exists a forward equivalence
between $Q_{I_{j+i}}^{e_i}$ and $Q_{I_{j{\geq}1}}^{e_0}$, and the
result holds.

If $ q^{e_*}_{u+1} = \delta(q_u^{e_*},(w(u+1),c_{u+1} {\geq} 0))$ and
$q^{e_*}_{u+1}$ $\in$ $Q_{I_0}^{e_*}$ then, since $A^{e_0}$ and
$A^{e_i}$ are communication stable, there exists $q^{e_i}_{u+1}\in
Q_{I_{c_{u+1}}}^{e_i}$ with $q^{e_i}_{u+1} = \delta(q_u^{e_i},w(u+1))$
and $q^{e_i}_{u+1}$ is isomorphic to $q_{u+1}^{e_*}$. Consider the
part of $\pi^{e_*}$ that stay in $Q_{I_0}^{e_*}$, and two states
$q^{e_*}_{l {\geq} u+1}$, $q^{e_*}_{l+1}$ with $q^{e_*}_{l+1} =
\delta(q^{e_*}_{l},(w(l+1),c_{l+1}))$. Let $q^{e_i}_{l}$ $\in$
$Q^{e_i}_{I_{z}}$ the state associated to $q^{e_*}_{l}$ in $\pi^{e_i}$
where $q^{e_i}_{l}$ is isomorphic to $q^{e_*}_{l}$, and let $z =
\sum_{k = 1}^{k = l}c_k$. The state corresponding to $q^{e_*}_{l+1}$
in $\pi^{e_i}$ is the state that is isomorphic to $q^{e_*}_{l+1}$ in
$Q_{I_{z+c_{l+1}}}^{e_i}$. If $c_{l+1}=0$, it is obvious. Else, this
follows from the fact that the transition
$(q^{e_*}_{l},(w(l+1),c_{l+1}),q^{e_*}_{l+1})$ simulates the existence
of $c_{l+1}$ increments that are communication equivalent to
$Q_{I_0}^{e_0}$ and to $Q_{I_z}^{e_i}$. Let $q_k^{e_*}$ be the last
state of $\pi^{e_*}$ that belong to $Q_{I_0}^{e_*}$, and $q_k^{e_i}$
its corresponding state in $\pi^{e_i}$. If $q_k^{e_*}=q_n^{e_*}$, then
the result holds. Otherwise, consider the transition
$(q^{e_*}_{k},(w(k+1),c_{k+1}),q^{e_*}_{k+1})$. If $c_{k+1} = 0$, then
$q_k^{e_i}$ $\in$ $Q_{I_{i}}^{e_i}$ . There exists a forward
equivalence between states of $Q_{I_{i}}^{e_i}$ and of
$Q_{I_{0}}^{e_0}$, and the result holds. If $c_{k+1} > 0$, then
$q_k^{e_i}$ $\in$ $Q_{I_{i-{c_{k+1}}}}^{e_i}$ and $q_{k+1}^{e_*}$
$\in$ $Q_{I_{m > 0}}^{e_*}$. Due to the communication equivalence
property, there exists a transition
$(q^{e_i}_{k},w(k+1),q^{e_i}_{k+1})$, where $q^{e_i}_{k+1}$ $\in$
$Q_{i+m}^{e_i}$ and $q^{e_i}_{k+1}$ is isomorphic to
$q^{e_*}_{k+1}$. Since states of $Q_{I_{i+m}}^{e_i}$ and of
$Q_{I_{m}}^{e_0}$ are in forward equivalence, the result holds.

\item

We prove that for each $i~{\geq}~0$, $w=w(1){\dots}w_n$ $\in$
$L(A^{e_i})$, then there exists $w_c$ in $L(A_c^{e_*})$ such that
$P(w_c) = (w,b {\leq} i)$. The result is direct if $i =
0$. We now suppose $i>0$.

Consider the unique accepting run $\pi^{e_i} =
q_0^{e_i}q_1^{e_i}q_2^{e_i}{\dots}q_n^{e_i}$ on $w$ in $A^{e_i}_c$. We
show that there exists an accepting run $\pi^{e_*} =
q_0^{e_*}q_1^{e_*}q_2^{e_*}{\dots}q_n^{e_*}$ on $w_c$ in $A^{e_*}$.

Let $q_0^{e_i}q_1^{e_i}q_2^{e_i}{\dots}q_u^{e_i}$ be the part of the
run that stay in $Q_H^{e_i}$. Since $Q_H^{e_i}$ and $Q_{H}^{e_0}$ are
isomorphic, the corresponding states in $A^{e_*}$ are
$q_0^{e_*},q_1^{e_*},q_2^{e_*},{\dots},q_u^{e_*}$, where for each $j$
$\in$ ${\lbrack}0{\dots}i{\rbrack}$, $q_j^{e_i}$ and $q_j^{e_*}$ are
the corresponding states by the isomorphism relation. If $q^{e_*}_u =
q^{e_*}_n$ or if the state that follows $q_u^{e_i}$ is a state of
$Q_{T_f}^{e_i}$, then the result holds.

Assume now that $q^{e_i}_{u+1} = \delta(q^{e_u}_{i},w(u+1))$ and that
$q^{e_i}_{u+1}$ $\in$ $Q_{I_{l{\geq}i}}^{e_i}$ then, since $Q_H^{e_0}$
and $Q_H^{e_i}$ are communication stable, their exists by construction
a transition $(q_{u}^{e_*},(w(u+1),i),q_{u+1}^{e_*})$, where
$q^{e_*}_{u+1}$ is the state isomorphic to $q_{u+1}^{e_i}$ in
$Q_{l-i}^{e_*}$. By definition there exists a forward equivalence
between $Q_{I_{l}}^{e_i}$ and $Q_{I_{l-i}}^{e_0}$, and the result holds.

If $q^{e_i}_{u+1} = \delta(q^{e_i}_{u},w(u+1))$ and that
$q^{e_i}_{u+1}$ $\in$ $Q_{I_{c < i}}^{e_i}$ then, since $Q_H^{e_0}$
and $Q_H^{e_i}$ are communication stable, their exists a transition
$(q_{u}^{e_*},(w(u+1),c),q_{u+1}^{e_*})$, where $q^{e_*}_{u+1}\in
Q_{I_0}^{e_*}$, and $q^{e_*}_{u+1}$ is isomorphic to
$q_{u+1}^{e_i}$. Consider now the part of $\pi^{e_i}$ that stays in
$\cup_{b=c}^{b=i-1}Q^{e_i}_{I_b}$.  Takes two states $q^{e_i}_{l}$
$\in$ $Q_{I_{l}}^{e_i}$ and $q^{e_i}_{l+1}$ $\in$ $Q_{I_{l+u}}^{e_i}$
such that $q^{e_i}_{l+1} = \delta(q^{e_i}_{l},w(l+1))$ and let
$q^{e_*}_{l}$ $\in$ $Q^{e_*}_{I_{0}}$ be the corresponding state of
$q^{e_i}_{l}$ $\in$ $\pi^{e_*}$, by construction there exists a
transition $(q_l^{e_*},(w(l+1),u),q_{l+1}^{e_*})$ in $\delta^{e_*}$
with $q_{l+1}^{e_*}\in Q_{I_0}^{e_*}$ and
$(q_{l+1}^{e_*},q_{l+1}^{e_i})~\equiv_{e_*,e_i}$. Let $q_k^{e_i}$
$\in$ $Q_{I_{z<i}}^{e_i}$ be the last state of $\pi^{e_i}$ in
$\cup_{b=c}^{b=i-1}Q^{e_i}_{I_b}$, and $q_k^{e_*}$ its isomorphic
state in $Q_{I_{0}}^{e_*}$. Let
$(w(1),c_1)(w(2),c_2){\dots}(w(k),c_k)$ be the part of $w_c$ that have
been read between $q_0^{e_*}$ and $q_k^{e_*}$.  We pose $s = \sum_{i =
1}^{i=k}c_k $. It is easy to see that $s = z$. If $q_k^{e_i} =
q_n^{e_i}$ or $q_{k+1}^{e_i}$ $\in$ $Q_{T_f}^{e_i}$, then the result
holds. Otherwise, there exists a transition
$(q^{e_i}_k,(w(k+1),q_{k+1}^{e_i})$ with $q_{k+1}$ $\in$
$Q_{I_{i+l}}^{e_i}$. By construction, there exists a transition
$(q^{e_*}_{k},(w(k+1),i-z),q^{e_*}_{k+1}$ with $q^{e_*}_{k+1}$ the
state isomorphic to $q^{e_i}_k$ in $Q_{I_{l}}^{e_0}$. Due to the
forward equivalence between $Q_{I_{i+l}}^{e_i}$ and $Q_{I_{l}}^{e_0}$,
the result holds.
\end{enumerate} 
\end{proof}

Theorem \ref{th-algo-count} shows that for each $w$ $\in$ $L(A^{e_i})$
and $w$ $\not\in$ $L(A^{e_{j<i}})$, there exists a word $w_c$ $\in$
$A^{e_*}_c$ such that $P(w_c) = (w,i)$.

Theorem \ref{th-algo-count} implies the correctness of algorithm
\ref{closure_algo_1}.

\begin{corollary}
\label{corollary-count}
Let $\widehat{A^{e^*}}$ be the finite-word automaton obtained by
applying algorithm \ref{closure_algo_1} to $A^{e_0}$, we have that
$L(\widehat{A^{e_*}}) = L(A^{e_*})$.
\end{corollary}

\begin{proof}
Let $A^{e_*}_c$ be the finite-word counter automaton obtained by
applying algorithm \ref{closure_algo_2} to $A^{e_0}$. We have that
$L_{\Sigma}(A^{e_*}_c) = L(\widehat{(A^{e_*}})$. For each $w$ $\in$
$L(\widehat{A^{e_*}})$, $\exists$ $w_c,i$ such that $w_c$ $\in$
$L(A_c^{e_*})$ and $P(w_c)=(w,i)$. By theorem \ref{th-algo-count},
one has that $w\in L(A^{e_i})$. The other direction follows by
noticing that for each pair $(w,i)$ with $w$ $\in$ $L(A^{e_i})$,
there exists $w_c,j~{\leq}~i$ with $w_c$ $\in$ $L(A_c^{e_*})$,
and $P(w_c)=(w,j)$, by construction $w$ $\in$ $L(\widehat{(A^{e_*}})$.
\end{proof}

\input{weak-extra}

==> figs/extrapolation.tex <==
\section{An Extrapolation Step for Sequence of Automata}
\label{extrap-1}

Consider the automaton $A^{e_0}$ of the sequence to which the
extrapolation step described at the end of Section \ref{increments}
can be applied. Following definitions \ref{def-incr-larger1}, the
state set $Q^{e_0}$ of $A^{e_0}$ can be decomposed into a head part
$Q_H^{e_0}$, a series of $k$ increments $Q_{I_0}^{e_0}, \ldots,
Q_{I_{k-1}}^{e_0}$, and a tail end part $Q_{T_f}^{e_0}$. Repeatedly
applying the extrapolation step described at the end of Section
\ref{increments} generates an infinite sequence of automata
$A^{e_0}A^{e_1},A^{e_2}{\dots}$ that grows incrementally, and such
that (1) for each $j$ $\in$ $0~{\leq}~j~{\leq}~k$, $A^{e_j} =
(Q^{e_j}, \Sigma, q_0^{e_j}, \delta^{e_j}, F^{e_j})$, (2) for each $i
> 0$, $Q_H^{e_i}$ is communication stable with $Q_H^{e_0}$, and (3)
for each $i > 0$, $Q_{I_0}^{e_i}$ is communication equivalent to
$Q_{I_0}^{e_0}$. Our goal is to build a single automaton that captures
the behavior of the automata in this sequence,
i.e. $A^{e_*}={\bigcup}_{i{\geq}0}A^{e_i}$. We will develop separated
solutions for finite-word and B\"uchi weak automata.

\subsection{The Finite Word Case}
\label{extra}

We aim at computing a finite representation of $A^{e_*}$ from a
sequence of finite-word automata. The idea is to build $A^{e_*}$ from
$A^{e_0}$ by adding new transitions that simulate the existence of
additional increments.

Consider a transition labeled by a symbol $a$ that goes from a state
$x$ of $Q_{I_0}^{e_0}$ to a state $x'$ of $Q_{I_3}^{e_0}$, and a
transition labeled by $b$ that goes from a state $y$ of $Q_H^{e_0}$ to
a state $y'$ of $Q_{I_2}^{e_0}$. Consider now $A^{e_1}$, which is
incrementally larger than $A^{e_0}$. Since, the increment
$Q_{I_0}^{e_1}$ added between $A^{e_0}$ and $A^{e_1}$ is also
communication equivalent to $Q_{I_0}^{e_0}$ there must exist a
transition labeled by a symbol $a$ from the state of $Q_{I_0}^{e_1}$
that is isomorphic to $x$ to the state that is isomorphic to $x'$ in
$Q_{I_2}^{e_1}$. We do not want to add the new increment, but we can
simulate its existence by adding a transition labeled by a symbol $a$
from the state $x$ of $Q_{I_0}^{e_0}$ to the state isomorphic to $x'$
in $Q_{I_2}^{e_0}$. The same principle can be repeated if we add two
or three increments. Simulating more than three increments can be done
by adding transitions to increment $Q_{I_0}^{e_0}$. Due to the
communication equivalence property, a transition labeled by $b$ must
also be added between the state $y$ of $Q_H^{e_0}$ and the state that
is isomorphic to $y'$ in $Q_{I_1}^{e_0}$. The situation is illustrated
in Figure \ref{extra-algo2}, where the dashed transitions are the
transitions added during the extrapolation process.

\begin{figure}
\begin{center}
\input{figs/figs/extra1.pstex_t}
\end{center}
\caption{Illustration of the extrapolation algorithm for
finite-word automata with the addition of counters.
\label{extra-algo2}
}
\end{figure}

Formally, the finite-word automaton $A^{e_*}$ can be built from $A^{e_0}$ by
adding transition with the following algorithm.

\begin{algo}
\label{closure_algo_1}
Consider the finite word automaton $A^{i+k} = A^{e_0} = (Q^{e_0},
\Sigma, q_0^{e_0},$\\$\delta^{e_0}, F^{e_0})$. We build a finite word
automaton ${A^{e_*}} = (Q^{e_*}, \Sigma, q_0^{e_*},
\delta^{e_*}, F^{e_*})$, where $Q^{e_*} = Q^{e_0}$, $q_0^{e_*} =
q_0^{e_0}$, and $F^{e_*} = F^{e_0}$. Each state $q^{e_*}$ of
${A^{e_*}}$ is associated to exactly one state $q^{e_0}$ of
$A^{e_0}$ by a relation $\equiv~{\subseteq}~Q^{e_0} \times
Q^{e_*}$. Moreover $Q^{e_*}$ can be decomposed into
$Q_H^{e_0}~{\equiv}~Q_H^{e_*}$, a series of $k$ increments
$Q_{I_0}^{e_0}~{\equiv}~Q_{I_0}^{e_*}, \ldots,
Q_{I_{k-1}}^{e_0}~{\equiv}~Q_{I_{k-1}}^{e_*}$, and a final tail part
$Q_{T_f}^{e_0}~{\equiv}~Q_{T_f}^{e_*}$. The transition relation
$\delta^{e_*}$ is built in the following way. For each transition
$(q_x^{e_0},a,q_y^{e_0})$ in $A^{e_0}$, there exists a transition
$(q_x^{e_*},a,q_y^{e_*})$ in $A^{e_*}$ with $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$. For each state $q \in
Q_{H}^{e_0} \ {\cup} \ Q_{I_0}^{e_0}$ and for every $a \in \Sigma$,
\begin{quote}
If $\delta^{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}^{e_0}$, $1\leq j \leq k -1$, then for each
increment $Q_{I_{\ell}}^{e_*}$ with $0\leq \ell < j$, there is a
transition $(q_x^{e_*},a,(q_y^{e_*})')$ in ${A^{e_*}}$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, and $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0} \equiv q_y^{e_*}$.
\end{quote}
\end{algo}

The algorithm exploits the fact that the added increments must be
isomorphic and communication equivalent to $Q^{e_0}_{I_0}$. It is
fairly easy to see all computations generated using the added
transitions correspond to a computation of some $A^{e_i}$, and that
all the computations are considered. A formal proof of the correctness
of algorithm \ref{closure_algo_1} will be given in Section
\ref{count}.

\input{weak-extra}

==> figs/implementation.tex <==
\section{Implementation Issues}
\label{imple}

Implementing the techniques presented in this paper requires
potentially costly composition and determinization procedures. In
this section, we describe algorithmic improvements that, in several
practical cases, decrease substantially the cost of these procedures.

\subsection{Dominance}

Looking at the states generated during the determinization steps of an
element in the sampling sequence, it appeared that they corresponded
to large, but vastly redundant, sets of states of the nondeterministic
automaton. This redundancy is due to the fact that there are frequent
inclusion relations between the languages accepted from different
states of the automaton. We formalize this observation with the
following notion of {\em dominance}, similar to the concept used in
the ordered automata of~\cite{WB00,BW02}.

\begin{definition}
Given a nondeterministic finite automaton $A$, and two states $q_1$
and $q_2$ of $A$. We say that a state $q_1$ {\em dominates} a state
$q_2$ (denoted $q_1 \geq q_2$) if $L(A_{q_2}) \subseteq L(A_{q_1})$.
\end{definition}

Clearly, when applying a subset construction, each subset that is
generated can be simplified by eliminating dominated states. However,
in order to use this, we need to be able to efficiently compute the
dominance relation.

First we remark that this can be done by adapting an existing
algorithm~\cite{HHK95}. This algorithm has a time complexity of
$O(M{\times}N)$, where $M$ and $N$ are respectively the number of
states and transitions of the automaton. The space complexity is
$O(M^2)$.

In our context, there is a way to improve the computation. The idea is
to approximate the dominance relation of an automaton in the sequence
by using the dominance relation of the often smaller automata that
participated to its creation.

Consider, as an example, two transducers $T^1$, and $T^2$, and an
automaton $A$ on $\Sigma$. It is easy to see that if $q_1 \geq q'_1$
in $T_1$, $q_2 \geq q'_2$ in $T_2$, and $q_3 \geq q'_3$ in $A$, then
$(q_1,q_2) \geq (q'_1,q'_2)$ in $T_2 \circ T_1$ and $(q_1,q_3) \geq
(q'_1,q'_3)$ in $T_1(A)$.

\subsection{Nonreflexive Composition}

Consider a transducer $T_0~=~T~\cup~T_{id}$, and an exponential
sampling sequence $s_i = 2^i$ for all $i > 0$. Any transducer
$(T_0)^{s_j}$, with $j > 1$, can easily be computed as the sequential
composition of $(T_0)^{s_{j-1}}$ with itself.

In experiments, one observes that computing the deterministic form of
$(T_0)^{s_j}$, where $j > 1$ is usually much more costly than
computing $(T)^{s_j}$. The computation of $(T_0)^{s_j}$ can then be
made more efficient by using the formula $(T_0)^{s_j} =
((T_0)^{s_{j-1}} \circ (T)^{s_{j-1}}) \,\cup\, (T_0)^{s_{j-1}}$
instead of $(T_0)^{s_j} = (T_0)^{s_{j-1}} \circ (T_0)^{s_{j-1}}$. The
generalization to $(T_0)^{s_j}(A)$ is direct.

\subsection{Removing States}

The composition of two automata is an automaton that can contains
states whose accepted language is empty. Removing those states has two
main advantages: (1) it can reduce the number of states of the
deterministic automaton, and (2) it can reduce the number of states
needed to create one state of the deterministic automaton.

Computing the set of states whose language is empty can be done in
linear time for both finite-word and B\"uchi weak automata.






==> figs/improv-counting.tex <==
\section{A Preciseness Criterion for Integer and Reals systems}

The idea is to add on extra variable.

Show how it works.


==> figs/increments.tex <==
\section{Detecting increments}
\label{increments}

We consider a sequence $A^1, A^2, A^3, \ldots$ of finite-word
(resp. B\"uchi weak) automata, which are assumed to be deterministic
and minimal. Our goal is to determine whether, for sufficiently large
$i$, the automaton $A^{i+1}$ differs from $A^i$ by some additional
constant finite-state structure. Our strategy, consists in comparing a
finite number of successive automata until a suitable increment can be
detected.

For each $i > 0$, let $A^i = (Q^i, \Sigma, q_0^i, \delta^i, F^i)$.  In
order to identify common parts between $A^i$ and $A^{i+1}$, we
consider two equivalence relations between their states:

\begin{itemize}
\item The {\em forward equivalence relation\/} $E^i_f \subseteq
Q^i \times Q^{i+1}$ is such that
$(q,q')\in E^i_f$ iff the language accepted from $q$ in $A^i$ is
identical to the language accepted from $q'$ in $A^{i+1}$;
\item The {\em backward equivalence relation\/} $E^i_b \subseteq
Q^i \times Q^{i+1}$ is such that
$(q,q')\in E^i_b$ iff the language accepted by $A^i$
with $q$ as final state is identical to the language accepted
by $A^{i+1}$ with $q'$ as final state.
\end{itemize}

Since we are dealing with deterministic minimized automata, the {\em
forwards equivalence relation} $E^{s_i}_f$ is one-to-one (though not
total), and can easily be computed by partitioning the states of the
joint automaton $(Q^{s_i} \cup Q^{s_{i+1}}, \Sigma, q_0^{s_i},
\delta^{s_i} \cup \delta^{s_{i+1}}, F^{s_i} \cup F^{s_{i+1}})$
according to their accepted language. For finite-word automata, this
operation is easily carried out by Hopcroft's finite-state
minimization procedure~\cite{Hop71}. In the case of B\"uchi weak
deterministic automata, one use L{\"o}ding's algorithm
\cite{Loe01}. The automata being reduced and deterministic, the
parts of $A_0^{s_{i}}$ and $A_0^{s_{i+1}}$ linked by $E^{s_i}_f$ are
isomorphic, incoming transitions being ignored.

Due to canonicity, the {\em backwards equivalence} $E^{s_i}_b$ can be
computed by forward propagation, starting from the pair $(q_0^{s_i},
q_0^{s_{i+1}})$, and exploring the parts of the transition graphs of
$A^{s_{i}}$ and $A^{s_{i+1}}$ that are isomorphic to each other, the
transitions leaving these parts being ignored.

We are now able to define our notion of finite-state ``increment''
between two successive automata, in terms of the relations
$E^{s_i}_f$ and $E^{s_i}_b$.

\begin{definition}
\label{def-incr-larger1}
The automaton $A^{i+1}$ is\/ {\em incrementally larger} than $A^i$ if
the relations $E^i_f$ and $E^i_b$ cover all the states of $A^i$. In
other words, for each $q \in Q^i$, there must exist $q' \in Q^{i+1}$
such that $(q, q') \in E^i_f \cup E^i_b$.
\end{definition}

If  $A^{s_{i+1}}$ is incrementally larger than
$A^{s_{i}}$, the increment consists of the states that are matched
neither by  $E^{s_i}_f$, nor by $E^{s_i}_b$. 

\begin{definition}
\label{def-incr-larger2}
If $A^{i+1}$ is incrementally larger than $A^{i}$, then
the set $Q^{i}$ can be partitioned into $\{ Q_b^i, Q_f^i \}$,
such that
\begin{itemize}
\item The set $Q_f^i$ contains the states $q$ covered by $E^i_f$,
i.e., for which there exists $q'$ such that $(q, q') \in E^i_f$;
\item The set $Q_b^i$ contains the remaining states.
\end{itemize}
The set $Q^{i+1}$ can now be partitioned into
$\{ Q_H^{i+1}, Q_{I_0}^{i+1}, Q_T^{i+1} \}$, where
\begin{itemize}
\item The\/ {\em head part} $Q_H^{i+1}$ is the image by $E^{i}_b$
of the set $Q_b^{i}$;
\item The\/ {\em tail part} $Q_T^{i+1}$ is the image by $E^{i}_f$
of the set $Q_f^{i}$, dismissing the states that belong to
$Q_H^{i+1}$ (the intention is to have an unmodified head part);
\item The\/ {\em increment} $Q_{I_0}^{i+1}$ contains the states
that do not belong to either $Q_H^{i+1}$ or $Q_T^{i+1}$.
\end{itemize}
\end{definition}


\begin{figure}
\centerline{\input{figs/increment1.pstex_t}}
\caption{Partitioning automata states.}
\label{fig-parts}
\end{figure}

Definitions \ref{def-incr-larger1} and \ref{def-incr-larger2} are
illustrated in Figure \ref{fig-parts}.

Our expectation is that, when moving from one automaton to the next
in the sequence, the detected increment will always be the same.
We formalize this property by the following definition.

\begin{definition}
\label{def-incr-seq}
The sequence of automata $A^{i}$, $A^{i + 1}$,
\ldots, $A^{i + k}$\/ {\em grows incrementally} if
\begin{itemize}
\item for each $j \in [0, k-1]$, $A^{i+j+1}$ is 
incrementally larger than $A^{i+j}$;
\item for each $j \in [1,k-1]$, the increment
$Q_{I_0}^{i+j+1}$ is the image by $E^{i+j}_b$ of the increment
$Q_{I_0}^{i+j}$.
\end{itemize}
\end{definition}


A direct consequence of Definition \ref{def-incr-seq} is that for each
$i$ in ${\lbrack}1{\ldots}k{\rbrack}$ we have that $Q_H^{s_{i}}$ is
isomorphic to $Q_H^{s_{i+1}}$ if not taking the outgoing
transitions into account. 

Consider a sequence $A^{i}$, $A^{i + 1}$,
\ldots, $A^{i + k}$ that grows incrementally.
The tail part $Q_T^{i+j}$ of $A^{i+j}$, $j \in
[2,\ldots,k]$, will then consist of $j-1$ copies of the increment
plus a part that we will name the {\em tail-end part\/}. Precisely,
$Q_T^{i+j}$ can be partitioned into $\{ Q_{I_1}^{i+j},
Q_{I_2}^{i+k}, \ldots, Q_{I_{j-1}}^{i+j}, Q_{T_f}^{i+j} \}$,
where
\begin{itemize}
\item for each $\ell \in [1, \ldots, j-1]$, the {\em tail increment\/}
$Q_{I_\ell}^{i+j}$ is the image by the relation 
$E_f^{i+j-1} \circ E_f^{i+ j-2} \circ \cdots
\circ E_f^{i+j-\ell}$
of the ``head'' increment $Q_{I_0}^{i+j-\ell}$, where ``$\circ$''
denotes the composition of relations;
\item the {\em tail-end set\/} $ Q_{T_f}^{i+j}$ contains the
remaining elements of $Q_T^{i+j}$.
\end{itemize}

\begin{figure}
\begin{center}
%\includegraphics{figs/increment2.pstex_t}
\input{figs/increment2.pstex_t}
\end{center}
\caption{Automata in an incrementally growing sequence.}
\label{figure2}
\end{figure}
The situation is illustrated in Figure~\ref{figure2}.\\

Focusing on automaton $A^{s_{i + k}}$ in a sequence of incrementally
growing automata, its head increment $Q_{I_0}^{s_{i + k}}$ and all its
tail increments $Q_{I_\ell}^{s_{i+k}}$, $\ell \in [1,k-1]$ appearing
in its tail part $Q_T^{s_{i + k}}$ are images of the increment
$Q_{I_0}^{s_{i+1}}$ by a combination of forward and backward
equivalences. Thus, the transition graphs internal to all increments
are isomorphic to that of $Q_{I_0}^{s_{i+1}}$, and hence are
isomorphic to each other.

Our intention is to extrapolate the last automaton of an incrementally
growing sequence of automata by adding more increments, following a
regular pattern. In order to do this, we need to compare the
transitions leaving different increments.

\begin{definition}
\label{def-equiv-inc}
Let $A^{i + k}$ be the last automaton of an incrementally
growing sequence, let $Q_{I_0}^{i + k}, \ldots, Q_{I_{k-1}}^{i
+ k}$ be the isomorphic increments detected within $A^{i +
k}$, and let $ Q_{T_f}^{i+k}$ be its tail-end set. Then, an
increment $Q_{I_\alpha}^{i + k}$ is said to be\/ {\em communication
equivalent} to an increment $Q_{I_\beta}^{i + k}$ iff, for each
pair of corresponding states $(q,q')$, $q \in Q_{I_\alpha}^{i +
k}$ and $q' \in Q_{I_\beta}^{i + k}$, and $a \in
\Sigma$, we have that, either
\begin{itemize}
\item
$\delta(q,a) \in Q_{I_\alpha}^{i + k}$ and  
$\delta(q',a) \in Q_{I_\beta}^{i + k}$, hence leading to
corresponding states by the existing isomorphism, 
\item
$\delta(q,a)$ and  $\delta(q',a)$ are both undefined, 
\item
$\delta(q,a)$ and  $\delta(q',a)$ both lead to the same state of 
the tail end $Q_{T_f}^{i+k}$, or
\item
there exists some $\gamma$ such that $\delta(q,a)$ and
$\delta(q',a)$ lead to corresponding states of respectively 
$Q_{I_{\alpha+\gamma}}^{i + k}$ and $Q_{I_{\beta+\gamma}}^{i + k}$.
\end{itemize}
\end{definition}

We also need to compare the transitions leaving the head part of
different automata in the sequence.

\begin{definition}
\label{communication_stable}
Let $A_{s_{i+k-1}}$ and $A_{s_{i+k}}$ be the two last elements of an
incrementally growing sequence of automata, let $Q_{I_0}^{i + k},
\ldots, Q_{I_{k-1}}^{i + k}$ (resp. $Q_{I_0}^{i + k-1}, \ldots,
Q_{I_{k-1}}^{i + k-2}$) and $Q_{T_f}^{i+k}$ (resp. $Q_{T_f}^{i+k-1}$)
be respectively the isomorphic increments, and the tail-end set of
$A^{s_{i+k}}$ (resp.  $A^{s_{i+k-1}}$). Let also $Q_H^{s_{i + k -1}}$
and $Q_H^{s_{i + k}}$ be respectively the head parts of
$A_{s_{i+k-1}}$ and $A_{s_{i+k}}$. The head parts $Q_H^{s_{i + k -1}}$
and $Q_H^{s_{i + k}}$ are {\em communication stable} iff for each pair
of corresponding states $(q, q')$, $q$ ${\in}$ $Q_H^{s_{i + k -1}}$
and $q'$ ${\in}$ $Q_H^{s_{i + k}}$, and for each $a$ ${\in}$
${\Sigma}{\times}{\Sigma}$, we have that, either

\begin{itemize}
\item 
$\delta^{s_{i+k-1}}(q,a)$ ${\in}$ $Q_H^{s_{i+k-1}} $ and
$\delta^{s_{i+k}}(q',a)$ ${\in}$ $Q_H^{s_{i+k}}$, are corresponding
states by the existing isomorphism,
\item
 $\delta^{s_{i+k-1}}(q,a)$ is a state $q_f$ of $Q_{T_f}^{s_{i+k-1}}$
 and $\delta^{s_{i+k}}(q',a)$ is a state $q'_f$ of
 $Q_{T_f}^{s_{i+k}}$, where $q_f$ and $q_f'$ are corresponding
 states by the existing isomorphism,
\item 
 $\delta^{s_{i+k-1}}(q,a)$ is a state $q_x$ of $Q_{I_x}^{s_{i+k-1}}$
 and $\delta^{s_{i+k}}(q',a)$ is a state $q'_{x}$ of
 $Q_{I_x}^{s_{i+k}}$, where $q_x$ and $q'_x$ are corresponding states
 by the existing isomorphism,
\item 
$\delta^{s_{i+k-1}}(q,a)$ and  $\delta^{s_{i+k}}(q',a)$ are both undefined.
\end{itemize} 
\end{definition}

The strongly connected components of the automata in an incrementally
growing sequence can be characterized by the following theorem.

\begin{theorem}
\label{composante-th}
Consider an incrementally growing sequence $A^{i}$, $A^{i + 1}$,
\ldots, $A^{i + k}$ of automata.  For $l$ $\in$
${\lbrack}i{\dots}k{\rbrack}$, each strongly connected components of
$A^{i+l}$ is entirely included in either $Q_H^{i+l}$,
$Q_{I_{0{\leq}k<l}}^{i+l}$, or $Q_{T_f}^{i+l}$.
\end{theorem}

\begin{proof}
Follows from Definition \ref{def-incr-seq} which ensures that (1) for
each transition $(q,a,q')$, if $q$ $\in$ $Q_{T_f}^{i+l}$ then $q'$
$\in$ $Q_{T_f}^{i+l}$, and (2) if $q$ $\in$ $Q_{I_{0{\leq}j<l}}$ then
$q'$ $\in$ $Q_{I_{j'{\geq}j}}^{i+l}~\cup~Q_{T_f}^{i+l}$.
 \end{proof}

Finally, we define the {\em communication diameter} of an automaton in
a sequence. This notion will be used in the extrapolation process
described in Section \ref{extrap-1}.

\begin{definition}
\label{communication-distance}
Consider an automaton $A^{i+j}$ in an incrementally growing sequence
of automata $A^{i}$, $A^{i + 1}$, \ldots, $A^{i + k}$. The {\em
communication diameter} of $A^{i+k}$ is the greatest integer
$d~{\leq}~j-1 $, such that there exists $q_1\in Q_H^{i+j}\cup
Q_{I_0}^{i+j}$ and $q_2\in Q_{I_d}^{i+j}$.
\end{definition}

In order to extrapolate $A^{i + k}$, i.e., to guess the value of $A^{i
+ k + 1}$, we simply insert an new increment between the head part of
$A^{i + k}$ and its head increment $Q_{I_0}^{i + k}$ and define the
transitions leaving it in order to make it communication equivalent to
$Q_{I_0}^{i + k}$.


==> figs/introduction.tex <==
\section{Introduction}

All the techniques that have been proposed for exploring infinite
state spaces, need a symbolic representation that can finitely represent
infinite sets of states. In early work on the subject, this
representation was domain specific, for example linear constraints for
sets of real vectors. For several years now, the idea that a generic
finite-automaton based representation could be used in many settings
has gained ground, starting with systems manipulating queues and
integers~\cite{WB95,BGWW97,WB98,BRW98}, then moving to parametric
systems~\cite{KMMPS97}, and, recently, reaching systems using real
variables~\cite{BBR97,BJW01}.

For exploring an infinite state space, one does not only need a
finite representation of infinite sets, but also techniques for
finitely computing the effect of an unbounded number of transitions.
Such techniques can be either domain-specific, or generic. Domain-specific
techniques exploit the specific properties and representations of the
domain being considered and were, for instance, obtained for queues
in~\cite{BG96,BH97}, for integers and reals
in~\cite{WB95,Boi98,BW02,BHJ03}, for pushdown system
in~\cite{FWW97,BEM97}, and for lossy channels in~\cite{AJ96}. Generic
techniques consider finite-automata representations and provide
algorithms that operate directly on this representation, mostly
disregarding the domain for which it is used.

Generic techniques appeared first in the context of the verification
of systems whose states can be encoded by {\em finite words}, such as
parametric systems. The idea used there is that a configuration being
a finite word, a transition relation is a relation on finite words, or
equivalently a language of pairs of finite words. If this language is
regular, it can be represented by a finite-state automaton, more
specifically a {\em finite-state transducer}, and the problem then
becomes the one of iterating such a transducer. Finite-state
transducers are quite powerful (the transition relation of a Turing
machine can be modeled by such a transducer), the flip side of the
coin being that their iteration is neither always computable, nor
regular. Nevertheless, there are a number of practically relevant
cases in which the iteration of finite-state transducers can be
computed and remains finite-state. Identifying such cases and
developing (partial) algorithms for iterating finite-state transducers
has been the topic, referred to as ``regular model checking'', of a
series of recent
papers~\cite{KMMPS97,BJNT00,JN00,Tou01,DLS01,AJNdo03,BHV04,VSVA04}.

The question that initiated the work presented in this article is,
whether the generic techniques for iterating transducers could be
fruitfully applied in cases of which domain specific techniques had
been exclusively used so far. In particular, one of our goals was to
iterate finite-state transducers representing arithmetic relations
(see~\cite{BW02} for a survey). Beyond mere curiosity, the motivation
was to be able to iterate relations that are not in the form required
by the domain specific results, for instance disjunctive
relations. Initial results were very disappointing: The transducer for
an arithmetic relation as simple as $(x,x+1)$ could not be iterated by
existing generic techniques. However, looking for the roots of this
inapplicability through a mix of experiments and theoretical work, and
taking a pragmatic approach to solving the problems discovered, we
were able to develop an approach to iterating transducers that easily
handles arithmetic relations, as well as many other
cases. Interestingly, it is by using a tool for manipulating automata
(LASH~\cite{LASH}), looking at examples beyond the reach of manual
simulation, and testing various algorithms that the right intuitions,
later to be validated by theoretical arguments, were
developed. Implementation was thus not an afterthought, but a central
part of our research process.

The general approach that has been taken is similar to the one
of~\cite{Tou01} in the sense that, starting with a transducer $T$, we
compute powers $T^i$ of $T$ and attempt to generalize the sequence of
transducers obtained in order to capture its infinite union. This is
done by comparing successive powers of $T$ and attempting to
characterize the difference between powers of $T$ as a set of states
and transitions that are added. If this set of added states, or {\em
increment}, is always the same, it can be inserted into a loop in
order to capture all powers of $T$. However, for arithmetic
transducers comparing $T^i$ with $T^{i+1}$ did not yield an increment
that could be repeated, though comparing $T^{2^i}$ with $T^{2^{i+1}}$
did. So, a first idea we used is not to always compare $T^i$ and
$T^{i+1}$, but to extract a sequence of samples from the sequence of
powers of the transducer, and work with this sequence of
samples. Given the binary encoding used for representing arithmetic
relations, sampling at powers of $2$ works well in this case, but the
sampling approach is general and different sample sequences can be
used in other cases. Now, if we only consider sample powers $T^{i_k}$
of the transducers and compute $\bigcup_k T^{i_k}$, this is not
necessarily equivalent to computing $\bigcup_i T^{i}$. Fortunately,
this problem is easily solved by considering the reflexive transducer,
i.e. $T_{0} = T\cup T_{id}$ where $T_{id}$ is the identity
transducer, in which case working with an infinite subsequence of
samples is sufficient.

Once the automata in the sequence being considered have been
constructed and compared, and that an increment corresponding to the
difference between successive elements has been identified, the next
step is to allow this increment to be repeated an arbitrary number of
times by incorporating it into a loop. There are some technical issues
about how to do this, but no major difficulty. Once the resulting
``extrapolated'' transducer has been obtained, one still needs to
check that the applied extrapolation is safe (contains all elements of
the sequence) and is precise (contains no more).  An easy to check
sufficient condition for the extrapolation to be safe is that it
remains unchanged when being composed with itself. Checking
preciseness is more delicate, but we have developed a procedure that
embodies a sufficient criterion for doing so. The idea is to check
that any behavior of the transducer with a given number $k$ of copies
of the increment, can be obtained by composing transducers with less
than $k$ copies of the increment. This is done by augmenting the
transducers to be checked with counters and proving that one can
restrict theses counters to a finite range, hence allowing
finite-state techniques to be used.

Taking advantage of the fact that our extrapolation technique works on
automata, not just on transducers, we consider computing reachable
states both by computing the closure of the transducer representing
the transition relation, and by directly operating on successive set
of states reachable from the set of initial states. The first approach
yields a more general object and is essential if one wishes to extend
the method to the verification of liveness properties
(\cite{BJNT00,BLW04b}), but the second is often less demanding from a
computational point of view and can handle cases that are out of reach
for the first. Preciseness is not always possible to check when
working with state sets rather than transducers, but this just amounts
to saying that what is computed is possibly an overapproximation of
the set of reachable states, a situation which is known to be
pragmatically unproblematic.

Going further, the problem of using regular model checking technique
for systems whose states are represented by infinite (omega) words has
been addressed. To avoid the-hard-to implement algorithms needed for
some operations on infinite-word automata, only omega-regular sets
that can be defined by weak deterministic B\"uchi
automata~\cite{MSS86} are considered. This is of course restrictive,
but as is shown in~\cite{BJW01}, it is sufficient to handle sets of
reals defined in the first-order theory of linear constraints over
integer and real variables. Moreover using such a representation leads
to algorithms that are very similar to the ones used in the
finite-word case, and allows us to work with reduced deterministic
automata as a normal form. Due to these advantages and properties, one
can show that the technique developed for finite words can directly be
adapted to weak deterministic B\"uchi automata up to algorithmic
modifications.

Our technique has been implemented in a library that relies and
extends the LASH package~\cite{LASH}. This implementation has been
tested on case studies coming from different applications.



==> figs/model.tex <==
\section{The (Omega-)Regular Model Checking Framework}
\label{model}

We use the {\em (omega-)regular model checking} framework
\cite{KMMPS97,WB98,BJNT00,BLW04a}.

\begin{definition}
A {\em system} is defined as a triple $M=(\Sigma,
{\phi}_I, R)$, where
\begin{itemize}
\item
$\Sigma$ is a finite alphabet over which the system configurations
are encoded as finite (resp. infinite) words;
\item
$\phi_I~{\subseteq}~\Sigma^*$
(resp. $\phi_I~{\subseteq}~\Sigma^{\omega}$) is a set of initial
configurations represented by a finite-word (resp B\"uchi weak
deterministic) automaton $A_{\phi_I}$ over $\Sigma$;
\item
$R~\subseteq~(\Sigma\times \Sigma)^*$
(resp. $R~\subseteq~(\Sigma\times \Sigma)^{\omega}$) is a
length-preserving regular (resp. omega weak) relation that models the
transition relation of the system and that is represented by a
finite-word (resp. B\"uchi weak deterministic) transducer $T$ over
$\Sigma\times \Sigma$.
\end{itemize}
\end{definition}

The (omega-)regular model checking framework is powerful enough to
encode configurations and transitions of a large class of systems
including parametric systems \cite{BJNT00,AJNdo03}, push-down systems
\cite{FWW97}, queue systems \cite{BG96,BGWW97,WB98}, systems with
integer or real variables \cite{ACHH95,WB00,BJW01,BW02}, or systems
that manipulate pointer variables \cite{BHMV05}.
 
Given a system $(\Sigma, {\phi}_I, R)$, we are interested in solving
two problems:

\begin{itemize}
\item
{\em Computing the reachable states:} the goal is to compute an
automaton $T^*(A_{\phi_I})$ representing $R^*(\phi_I)$. This
representation is useful to check whether some configuration in a set
${\phi}_{F}$ is reachable from $\phi_I$. This is done by checking whether
${\phi}_{F}~{\cap}~L(T^*(A_{\phi_I}))$ is empty or not.
\item
{\em Computing the transitive closure of $R$:} the goal is to
compute a transducer $T^*$ representing the reflexive and transitive
closure $R^*$ of $R$. This representation is useful to compute the
reachability set of states, or for finding cycles between reachable
system configurations~\cite{BJNT00,BLW04b}.
\end{itemize}

Those problems are in general undecidable, but semi-algorithms exist,
which can either be domain specific, or generic.  Domain-specific
solutions exploit the specific properties and representations of the
domain being considered. Generic solutions provide algorithms that
operate directly on the automata representation, mostly disregarding
the domain for which it is used. They can be divided in $4$
categories.
\begin{enumerate}
\item
{\em Collapsing techniques} \cite{BJNT00,DLS01,AJNdo03} are techniques
that attempt to compute a finite representation of $T^*$ by collapsing
its states according to {\em simulation relations}.
\item
{\em Abstraction techniques}~\cite{BHV04,BHMV05} use predicate
abstraction to compute an upper approximation of $T^{*}$ or
$T^{*}(A_{\phi_I})$.
\item
{\em Learning techniques}~\cite{HV04,VSVA04,VSVA05} use learning
algorithms to learn $L(T^{*})$ or $L(T^{*}(A_{\phi_I}))$.
\item
{\em Extrapolation/Widening techniques}~\cite{BJNT00,Tou01,Tou03}
compare the automata obtained after several iterations of $T$, or
several applications of $T$ to $A_{\phi_I}$, and try to automatically
guess the limit of the sequence.
\end{enumerate}
\section{An Extrapolation Technique}

In this article, we tackle both of the problems presented in Section
\ref{model} by an approach that consists in extrapolating a finite
sequence of automata. The idea is to approximates the limit of the
sequence by considering a sample part. This approximation is done by
comparing successive automata in the sampling sequence; identifying
the difference between these in the form of an ``increment'', and
extrapolating the repetition of this increment. Finally, checks are
applied to ensure that this extrapolation corresponds to the limit of
the sequence. Those checks depend of the application being considered.

The following lemma is useful to shows that, for problems outlined in
Section \ref{model}, the sampling sequence can be selected quite
arbitrarily.

\begin{lemma}
\label{lemma-sample1}
Let $R$ be a relation on an alphabet $\Sigma{\times}\Sigma$, and $R_0
= R \,\cup\, R_{id}$. If $s_1, s_2, \ldots$ is an infinite increasing
subsequence of the natural numbers, then $R^* = \bigcup_{k \geq 0}
(R_0)^{s_k}$ and, similarly, $R^*(\phi_I)= \bigcup_{k \geq 0}
(R_0)^{s_k} ({\phi}_I)$.
\end{lemma}

The lemma follows directly from the fact that for any $i\geq 0$, there
is an $s_k\in s$ such that $s_k > i$ and that, since $R_0$ is
reflexive, $(\forall j \leq i)(R_0^j \subseteq R_0^i)$ (resp
$(R_0^j(\phi_I) \subseteq R_0^i(\phi_I))$).

Thus, given a system $(\Sigma, {\phi}_I, R)$, we compute a transducer
$T_0$ representing $R \,\cup\, \it R_{id}$, and select a {\em sampling
sequence\/} $s= s_1,s_2,\ldots$. Computing $R^*$ (resp. $R^*(\phi_I)$)
then amounts to computing the limit of the sequence of automata
$(T_0)^{s_1}$, $(T_0)^{s_2}$, $(T_0)^{s_3}$, \ldots
(resp. $(T_0)^{s_1}(A_{\phi_I})$, $(T_0)^{s_2}(A_{\phi_I})$,
$(T_0)^{s_3}(A_{\phi_I})$, \ldots). 

The rest of this article is organized as follow. Section
\ref{increments} describes an algorithm for detecting increments
between automata in a finite sequence.  Section \ref{extrap-1}
presents an extrapolation algorithm. Section \ref{safe-precis}
introduces criteria for checking the correctness of the
extrapolation. Notes on the implementation and the experiments are
respectively reported in Sections \ref{imple} and \ref{expe}. A
conclusion is given in Section \ref{conclu}.



==> figs/precis.tex <==
\section{Safety and Preciseness}
\label{safe-precis}

After having constructed the extrapolation $A^{e_*}$ of a sequence
$A^1$, $A^2, \ldots$ of automata, it remains to check whether it
accurately corresponds to what we really intend to compute, i.e.,
$\bigcup_{i > 0} A^i$. This is done by first checking that the
extrapolation is {\em safe\/}, in the sense that it captures all
behaviors of $\bigcup_{i > 0} A^i$, and then checking that it is {\em
precise\/}, i.e. that it has no more behaviors than $\bigcup_{i > 0}
A^i$. We check both properties using sufficient conditions. We develop
separately these conditions for the two problems outlined in
Section~\ref{model}.

\subsection{Transitive Closure of a Relation}
\label{subsec-transd}

In this section, we consider $T^{e_*}$, the transducer obtained by
applying Algorithm \ref{closure_algo_1} or Algorithm
\ref{closure_algo_3} to the last transducer $T^{e_0}$ of an
incrementally growing sampling sequence of powers of a transducer $T$. By
construction $L(T^{e_*}) = L(\cup_iT^{e_i})$, where $T^{e_0} =
T^{i+k}$. For each $i > 0$, $T^{e_i}$ is the automaton obtained from
$T^{e_0}$ by adding $i$ increments communication equivalent to the
increment detected between $T^{i+k-1}$ and $T^{i+k}$.

We start with the following lemma.

\begin{lemma}
\label{safe-1}
Consider two reflexive finite-word (resp. B\"uchi weak) transducers
$T_1$ and $T_2$. If (1) $L(T_1)~{\subseteq}~L(T_2)$ and (2) $L(T_2
{\circ} T_2)~{\subseteq}~L(T_2)$, then $L(T_1^*)~{\subseteq}~L(T_2)$.
\end{lemma}

\begin{proof}
The proof is by induction on the powers of $T_1$,
i.e. $\forall~i~{\geq}~0$, $L(T^i_1)$~$\subseteq$~$L(T^{2})$. By
definition, the result holds for $T_1^0$ and $T_1$. Assume now that
$L(T_1^i)$ $\subseteq$ $L(T^{2})$. We have that $T_1^{i+1} = T_1^{i}
\circ T_1$ and thus $L(T_1^{i+1}) = L(T_1^{i} {\circ}
T_1)~{\subseteq}~L(T_2 {\circ} T_1)~\subseteq~L(T_2 {\circ}
T_2)~$\\${\subseteq}~L(T_2)$. The first inclusion holds because the
composition of transducers is a monotonic operation. The second
inclusion holds because of hypothesis (1), and the last inclusion is
justified by hypothesis (2).
\end{proof}

We now propose a sufficient condition for checking the safetiness of
our extrapolation. The condition is presented under the form of a
theorem.

\begin{theorem}
\label{safe1}
The transducer $T^{e_*}$ is a safe extrapolation of $T$ if $L(T^{e_*}
\circ T^{e_*}) \subseteq L(T^{e_*})$.
\end{theorem}

\begin{proof}
The proof is direct since hypothesis of Lemma \ref{safe-1} are
satisfied by posing $T_1 = T$, and $T_2 = T^{e_*}$.
\end{proof}

The previous criterion is only sufficient since there could exist two
words $w$ and $w'$ in $L(T^{e_*})$ such that $w$, $w'$ $\not\in$
$L(T^*)$ and $w~{\circ}~w'$ $\not\in$ $L(T^{e_*})$.

In practice, checking the condition expressed by Theorem \ref{safe1}
requires to complement $T^{e_*}$. This is immediate when considering
finite-word transducers. In the other case, $T^{e_*}$ is weak but
generally not deterministic. The solution we implemented consists in
determinizing $T^{e_*}$, and then checking whether the resulting
transducer is inherently weak. In the positive case, the transducer is
turned into a weak deterministic one, and easily
complemented. Otherwise, the test cannot be completed.  Another
solution would have been to implement the more general complementation
constructions given in \cite{KV01,CKV03,KV04,FKV04}.\\
\newline
\noindent
Determining whether the extrapolation is precise is a more difficult
problem for which we again provide a partial solution in the form of a
sufficient criterion. The ``preciseness'' problem amounts to proving
that any pair of words accepted by $T^{e_*}$, or equivalently by some
$T^{e_i}$, is also accepted by an iteration $T^j$ of the transducer
$T$. The idea is to check that this can be proved inductively. The
property is true by construction for the transducer $T^{e_0}$ from
which the extrapolation sequence is built. If we can also prove that,
if the property holds for all $T^{e_j}$ with $j<i$, then it also holds
for $T^{e_i}$, we are done. For this, we propose the following
condition.

\begin{equation}
\label{extra1}
 \forall w, {\forall} i >0 \
{\lbrack}w \in L(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w \in
L(T^{e_j}{\circ}T^{e_j'}){\rbrack}.
\end{equation}

To check Condition \ref{extra1}, we use automata with counters.
Consider $T^{e_*}_{c_1}$, $T^{e_*}_{c_2}$, and $T^{e_*}_{c_3}$ to be
three copies of the counter automaton obtained by applying Algorithm
\ref{closure_algo_2} or Algorithm \ref{closure_algo_4} to the
transducer $T^{e_0}$. We resort the following condition.

\begin{equation}
\label{equa-precis1}
L({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c (T_{c_2}^{e_*}
\circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*}).
\end{equation}

We have the following theorem.

\begin{theorem}
We have that $L({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c
(T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*})$
is satisfied iff for all $w$ on $(\Sigma {\times} \Sigma)$, for all $
i >0 \ {\lbrack}w \in L(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w
\in L(T^{e_j}{\circ}T^{e_j'}){\rbrack}$ is satisfied.
\end{theorem}

\begin{proof}
We prove the two directions.
\begin{enumerate}
\item
We show that if $ L({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c
(T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*})$,
then $\forall w, {\forall} i >0 \ {\lbrack}w \in L(T^{e_i}) \
{\Rightarrow} \ {\exists}j,j'<i, w \in
L(T^{e_j}{\circ}T^{e_j'}){\rbrack}$. If $w$ $\in$ $L(T^{e_i})$ and $w$
$\not\in$ $L(T^{e_{j<i}})$ then, by Theorem \ref{th-algo-count2},
there exists $w_c$ $\in$ $L(T_{c_1}^{e_*})$ such that $P(w_c) =
(w,i)$. Since Condition \ref{equa-precis1} holds, there exists $w_c'$,
$w_c''$ $\in$ $L(T^{e_*}_{c_1})$ such that $P(w_c') = (w',j)$, and
$P(w_c'') = (w'',j')$ with $j,j'<i$, and $w = w'~{\circ}~w''$. By
theorem \ref{th-algo-count1}, $w'$ $\in$ $L(T^{e_j})$ and $w''$ $\in$
$L(T^{e_{j'}})$.
\item
We show that if $\forall w, {\forall} i
>0 \ {\lbrack}w \in L(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w
\in L(T^{e_j}{\circ}T^{e_j'}){\rbrack}$, then
$L({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c (T_{c_2}^{e_*}
\circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*})$. We must show
that each word $w_c$ $\in$ $L(A^{e_*}_{c_1})$ with $P(w_c)=(w,i>0)$
can be obtained from two words $w_c'$ and $w_c''$ $\in$
$L(T^{e_*}_{c_1})$, where $P(w_c')=(w',l<i)$, $P(w_c'')=(w'',l'<i)$,
and $w = w'~{\circ}~w''$. By theorem \ref{th-algo-count1}
(resp. Theorem \ref{th-algo-count2}), $w$ $\in$ $T^{e_i}$. Since
Condition \ref{extra1} is satisfied, there exists $w'$ $\in$
$L(T^{e_{j<i}})$, and $w''$ $\in$ $L(T^{e_{j'<i}})$ with $w = w'
{\circ} w''$. By theorem \ref{th-algo-count2}, there exists also
$w_c'$, $w_c''$ $\in$ $L(A^{e_*}_c)$ with $P(w_c')=(w',l~{\leq}~j)$,
and $P(w_c'')=(w'',l'~{\leq}~j')$.
\end{enumerate}
\end{proof}

The remaining difficulty is to provide an algorithm for the operation
$\pi_{c_1 > c_2,c_3}$, and more generally for $\pi_{c_i >
c_{a1},{\dots},c_{ax}}$. Clearly, this is undecidable since we are
considering counter automata that handle at least two counters. We
again provide a partial solution to the problem.

We first remark that what we need to check is that, if the value of
$c_i$ is greater than $0$, then the differences between the value of
$c_i$ and the value of $c_{al}$ must be greater than $0$, for each
$1~{\leq}~l~{\leq}~x$.

In practice, we observed that the counters involved in a difference
are often incremented in a particular way. Those observations are
formalized by the following definition.

\begin{definition}
\label{synchro-count}
The counter automaton $A_c=(Q,\Sigma
{\times}{\lbrack}0{\dots}d{\rbrack}^n, q_0, \delta,F)$ is\/ {\em
synchronized} with respect to the counters $c_{i{\leq}n}$ and
$c_{j{\leq}n}$ if there exists $M > 0$ such that each $w_c \in L(A_c)$
can be accepted by a run $\pi$, each subrun $\sigma$ of which
satisfies $\Delta c_j(\sigma) < \Delta c_i(\sigma)$ $+$ $M$ if $\Delta
c_i(\pi) > 0$, where $\Delta c_l(\sigma)$ denotes the counter
increments applied to $c_l$ while following $\sigma$ on $w_c$.
\end{definition}

\begin{definition}
\label{counter-machine}
A counter automaton on an alphabet $\Sigma
{\times}{\lbrack}0{\dots}d{\rbrack}^n$ that accepts all the words on
$\Sigma {\times}{\lbrack}0{\dots}d{\rbrack}^n$ that satisfies
Definition \ref{synchro-count} for two counters $c_i$ and $c_j$ and a
born $M$ is called a {\em finite-word (resp. B\"uchi weak) counter
machine on $(c_i,c_j,M)$}.
\end{definition}


Given a counter automaton $A_c=(Q,\Sigma_a
{\times}{\lbrack}0{\dots}d{\rbrack}^n,q_0, \delta,F)$, it is easy
to compute a counter automaton $A_c'$ on
$\Sigma{\times}{\lbrack}0{\dots}d{\rbrack}^n$, where
$L(A_c')~{\subseteq}~L(\pi_{c_i > c_{a1},{\dots},c_{ax}}(A_c))$. The
idea is to impose a synchronization between the counters that need to
be compared. To do this, we fix a born $M>0$ and then construct $x$
counter machines $A_{c_i - c_{al}}$ on $(c_i,c_{al},M)$. We then take
the intersection between $A_c$ and the counter machines. Finally, we
compute the projection on $\Sigma{\times}{\lbrack}0{\dots}d{\rbrack}$
to get the final result.

We now give a procedure for checking Condition \ref{equa-precis1}. We
first compute ${\lbrack}T_{c_1}^{e_*} \cap_c (T_{c_2}^{e_*} \circ_c
T_{c_3}^{e_{*}}){\rbrack}$ using the constructions given in Section
\ref{counters}. We then apply two counter machines, one on
$(c_1,c_2,M)$ and one on $(c_1,c_3,M)$. We get a counter automaton
$A_c'$ whose transitions are labeled by elements of the alphabet
$\Sigma{\times}\Sigma\times{\lbrack}0{\dots}d{\rbrack}^3$. The labels
$(a,b,x,y,z)$ of the transitions of $A_c'$ are renamed into $(a,b,x)$,
creating a new counter automaton on the alphabet
$\Sigma{\times}\Sigma\times{\lbrack}0{\dots}d{\rbrack}$. The language
of this new structure can be compared with the one of $A^{e_*}_{c_1}$
using existing algorithms \ref{Hop71,Var95}. The implementation of
those algorithms require, in general, the complementation of the
automata whose languages are compared. This operation is conducted
with a procedure that is identical to the one used to check the
condition expressed by Theorem \ref{safe1}. It is worth mentioning
that, in practice, we choose the born $M$ to be a multiple of the
communication diameter of $T^{c_1}_{e_*}$. Finally note that, due to
the synchronization between counters, the preciseness criterion is
sufficient but not necessary.

\subsection{Limit of a Sequence of Reachable Sets}

In this section, we consider $A^{e_*}$ to be the automaton obtained by
applying Algorithm \ref{closure_algo_2} or Algorithm
\ref{closure_algo_4}) to the last automaton $A^{e_0}$ of an
incrementally growing subsequence $A$, $T(A)$, $(T)^2(A)$, $(T)^3(A)$,
, $\dots$ of automata, where $T$ is a reflexive transducer. By
construction $L(A^{e_*}) = L(\cup_iA^{e_i})$, where $A^{e_0} =
A^{i+k}$. For each $i>0$, $A^{e_i}$ is the automaton obtained from
$A^{e_0}$ by adding $i$ increments communication equivalent to the
increment detected between $A^{i+k-1}$ and $A^{i+k}$.

Following the same scheme as in Section \ref{subsec-transd}, we first
give a sufficient criterion for checking the safetiness of the
extrapolation. We then provide a criterion for checking preciseness.

\begin{lemma}
\label{safe-2}
Let $T$ be a reflexive transducer, and $A_1$ and $A_2$ be two
automata. If (1) $L(A_1)~{\subseteq}~L(A_2)$, and
$L(T(A_2))~\subseteq~L(A_2)$, then $L(T^*(A_1))~{\subseteq}~L(A_2)$.
\end{lemma}

\begin{proof}
We proof by induction that $\forall i$,
$L(T^{i}(A_1))~{\subseteq}~L(A_2)$.  If $i = 0$, then $L(T^{0}(A_1)) =
L(A_1)~{\subseteq}~L(A_2)$, the equality comes from the definition of
the identity relation, and the inclusion from hypothesis (1). Assume
now that $L(T^i(A_1))~{\subseteq}~L(A_2)$. We have that
$L(T^{i+1}(A_1)) =
L(T(T^i(A_1)))~{\subseteq}~L(T(A_2))~{\subseteq}~L(A_2)$. The first
inclusion stands because the composition is monotonic, and the second
because of hypothesis (2).
\end{proof}

\begin{theorem}
The automaton $A^{e_*}$ is a safe extrapolation of $T^*(A)$ if\\
$L(T(A^{e_*})~{\subseteq}~L(A^{e_*})$.
\end{theorem}

\begin{proof}
The proof is direct since the hypothesis of Lemma \ref{safe-2} are
satisfied by posing $A_1 = A$ and $A_2 = A^{e_*}$.
\end{proof}

We now give a preciseness criterion. The idea borrow on the one
developed in Section \ref{subsec-transd}. More precisely, the
preciseness problem amounts to show that each word accepted by
$A^{e_*}$ can be accepted by an automaton $T^i(A)$. This is true by
construction for the automaton $A^{e_0}$, if we can also prove that if
the property holds for $A^{e_j}$ with $j<i$ then it holds for
$A^{e_i}$, we are done. We propose the following condition.

\begin{equation}
\label{extra2}
{\forall} w, \forall i > 0
{\lbrack}w \in L(A^{e_i}) \Rightarrow \exists j < i, w \in
L(T(A^{e_j})){\rbrack}.
\end{equation}

Condition \ref{extra2} ensures that each word $w'\in L(A^{e_i})$ can
be obtained from a word $w$ in $A^{e_0}$ by applying $j<i$ times the
transition relation $T$, i.e. $w'=T^j(w)$.

Checking the satisfaisability of Condition \ref{extra2} is done with a
technique that is similar to the one developped in Section
\ref{subsec-transd}.

\begin{equation}
\label{equa-precise2}
L({\pi}_{c_1>c_2}{\lbrack}A^{e_*}_{c_1}\cap_c
T(A_{c_2}^{e_*}){\rbrack})= L(A_{c_1}^{e_*}).
\end{equation}

\begin{theorem}
We have that \label{extra2} ${\forall} w \in \Sigma^{*}({\mbox{resp. }}
\Sigma^{\omega}), \forall i > 0 {\lbrack}w \in L(A^{e_i}) \Rightarrow
\exists j < i, w \in L(T(A^{e_j})){\rbrack}$ is satisfied iff
$L({\pi}_{c_1>c_2}{\lbrack}A^{e_*}_{c_1}\cap_c
T(A_{c_2}^{e_*}){\rbrack})= L(A_{c_1}^{e_*})$ is satisfied.
\end{theorem}

\begin{proof}
We prove the two directions of the equivalence.
\begin{enumerate}
\item
If $L({\pi}_{c_1>c_2}{\lbrack}A^{e_*}_{c_1}\cap_c
T(A_{c_2}^{e_*}){\rbrack})= L(A_{c_1}^{e_*})$ then ${\forall} w,
\forall i > 0 {\lbrack}w \in L(A^{e_i}) \Rightarrow \exists j < i, w
\in L(T(A^{e_j})){\rbrack}$. If $w$ $\in$ $L(A^{e_i})$ and $w$
$\not\in$ $L(A^{e_{j<i}})$ then, by Theorem \ref{th-algo-count2},
there exists $w_c$ $\in$ $L(A^{e_*}_{c_1})$, such that $P(w_c) =
(w,i)$. Since Condition \ref{equa-precise2} holds, there exists $w_c'$
$\in$ $L(A^{e_*}_{c_1})$ and $(w',w))$ $\in$ $L(T)$, such that
$P(w_c') = (w',j < i)$. By Theorem \ref{th-algo-count1}, there exists
$w'$ $\in$ $L(A^{e_{j<i}})$.
\item
If ${\forall} w, \forall i > 0 {\lbrack}w \in L(A^{e_i}) \Rightarrow
\exists j < i, w \in L(T(A^{e_j})){\rbrack}$, then
$L({\pi}_{c_1>c_2}{\lbrack}A^{e_*}_{c_1}\cap_c
T(A_{c_2}^{e_*}){\rbrack})= L(A_{c_1}^{e_*})$. We must show that each
word $w_c$ $\in$ $L(A^{e_*}_{c_1})$ with $P(w_c) = (w,i)$, can be
obtained from the composition of $T$ with a word $w_c'\in$
$L(A^{e_*}_{c_1})$ such that $P(w_c')=(w',l<i)$. By Theorem
\ref{th-algo-count1}, $w$ $\in$ $L(A^{e_i})$. Since Condition
\ref{extra2} holds, there exists $w'$ $\in$ $L(A^{e_{j<i}})$, and a
pair $(w',w)$ $\in$ $L(T)$. By Theorem \ref{th-algo-count2}, there
exists also $w_c'$ $\in$ $L(A^{e_*}_{c_1})$ such that $P(w_c') =
(w',l~{\leq}~j)$, and $T(w') = w$.
\end{enumerate}
\end{proof}

Checking if $L({\pi}_{c_1>c_2}{\lbrack}A^{e_*}_{c_1}\cap_c
T(A_{c_2}^{e_*})_c{\rbrack})= L(A_{c_1}^{e_*})$ can be done by first
computing ${\lbrack}T(A_{c_2}^{e_*})_c \cap_c A^{e_*}_{c_1}{\rbrack}$
using the constructions given in Section \ref{counters}, and then
apply a counter machine on $(c_1,c_2,M)$. The labels $(a,x,y)$ of the
transitions of the result are then renamed into $(a,x)$. This allows a
comparison with the language of $A_{c_1}^{e_*}$, using the
implementation described at the end of Section \ref{subsec-transd}.

\subsection{Counter Machine}
\label{counters}

Given an alphabet $\Sigma_a {\times}{\lbrack}0{\dots}d{\rbrack}^n$ and
a tuple $(c_i,c_j,M)$, we aim to construct a finite-word counter
machine on $(c_i,c_j,M)$. It is easy to see that an empirical
construction can lead to an automaton whose number of states is of
$O(M^2)$. We propose here a machine whose size is of $O(M)$. This
machine is more expressive that the one described in Definition
\ref{synchro-count}. As this will be explained later, this additional
expressivity has no negative influence on the final result.

We denote by $v(c_i)$ and $v(c_j)$ the value of the counters $c_i$ and
$c_j$. The machine has $3{\times}M$ states: a state labeled by $v(c_i)
= v(c_j)$ for the case in where the value of $c_i$ is equal to the one
of $c_j$, $M-1$ states labeled by $v(c_j)=v(c_i)+l$ with $l$ $\in$
${\lbrack}1,{\dots},M-1{\rbrack}$ to check the synchronization when
$v(c_j)>v(c_i)$, $2{\times}M-1$ states labeled by $v(c_i)=v(c_j)+l$
with $l$ $\in$ ${\lbrack}1,{\dots},2{\times}M-1{\rbrack}$ to check the
synchronization when $v(c_i)>v(c_j)$. There is also an initial state
labeled by ``initial''. The accepting states are those labeled by
$v(c_i) = v(c_j)+l$ with $l$ $\in$
${\lbrack}1,{\dots},2{\times}M-1{\rbrack}$. The initial state is also
an accepting state.  Given a label
$w(x)=(a,c_{1x},{\dots},c_{ix},{\dots},c_{jx},{\dots},c_{nx})$ with
$a$ $\in$ $\Sigma$ and
$c_{1x},{\dots},c_{ix},{\dots},c_{jx},{\dots},c_{nx}$ $\in$
${\lbrack}0{\dots}d{\rbrack}$, we define $diff=c_{ix}-c_{jx}$. From a
state $v(c_i)=v(c_j)+l$ with $l$ $\in$
${\lbrack}-M+1,{\dots},M-1{\rbrack}$, if the machine follows a
transition labeled by $w(x)$, then it goes to a state
$v(c_i)=v(c_j)+l+diff$ if $l+diff$ $\in$
${\lbrack}-M+1,{\dots},M-1{\rbrack}$, or to the state labeled by
$v(c_i)=v(c_j)+M$ if $l+diff>M-1$. Otherwise the transition is not
defined. From the initial state, if the machine follows a transition
labeled by $w(x)$, then it goes to a state $v(c_i)=v(c_j)+l+diff$ if
$diff$ $\in$
${\lbrack}-M+1,{\dots}-1{\rbrack}~{\cup}~{\lbrack}1,{\dots},M-1{\rbrack}$,
or to the state $v(c_i)=v(c_j)+M$ if $diff>M-1$, or to the initial
state if $diff = 0$. From a state $v(c_i)=v(c_j)+l$ with $l$ $\in$
${\lbrack}M,{\dots},2{\times}M-1{\rbrack}$, the machine goes to
$c(v_i)=c(v_j)+M$ if $l-diff~{\leq}~M$, or to $v(c_i)=v(c_j)+l-diff$
if $l-diff$ $\in$
${\lbrack}M+1,{\dots},2{\times}M-1{\rbrack}$. Otherwise, the
transition is not defined.

Due to the synchronization, if the machine is in a state labeled by
$v(c_i)=v(c_j)+M$, then $v(c_i)>v(c_j)$. In this situation, only the
synchronization property needs to be checked. This is done by using
the states labeled by $v(c_i)=v(c_j)+l$, with $l$ $\in$
${\lbrack}M,{\dots},2{\times}M-1{\rbrack}$.

The main difference between the construction we proposed and an
empirical one is that our construction only check $\Delta c_j(\sigma)
< \Delta c_i(\sigma)$ $+$ $M$ when $v(c_i)=v(c_j)$, or when
$v(c_i)=v(c_j)+M$. Normally, this should be done for each state
labeled by $v(c_i)=v(c_j)+l$ with $l$ $\in$
${\lbrack}1,{\dots},M-1{\rbrack}$. This simplification leads to
situations in where runs satisfying $\Delta c_j(\sigma) < \Delta
c_i(\sigma)$ $+$ $2{\times}M$ can be accepted.

When moving from the finite word case to the $\omega$-word case, the
construction stays the same, and results in a weak B\"uchi
automaton. However, this machine cannot be turned to a weak
deterministic automaton. This means that each application of the
machine to a a weak deterministic B\"uchi automaton is followed by a
test to check if the result is still weak and deterministic.



==> figs/preli-old.tex <==
\section{Preliminaries}

In this section, we introduce the theoretical concepts that will be
used in the rest of this article.

\subsection{Automata}
\label{automata-intro}

A {\em finite word\/} $w$ over a finite alphabet $\Sigma$ is a finite
sequence of elements of $\Sigma$. An {\em infinite word \/}(or {\em
$\omega$-word\/}) $w$ over $\Sigma$ is a countably infinite sequence
of elements of $\Sigma$. The $i-th$ element (also called symbol) of
the sequence $w$ is denoted by $w(i)$.  The set of finite and infinite
words over $\Sigma$ are respectively denoted by $\Sigma^*$ and
$\Sigma^{\omega}$. A language on $\Sigma$ is a set of words over
$\Sigma$. The complement of $L$ is defined by
$\bar{L}={\lbrace}w~|~w\notin L{\rbrace}$. Given two languages $L_1$
and $L_2$, their union and intersection are respectively defined by
$L_1\cup L_2={\lbrace}w~|~w\in L_1\mbox{ or } w\in L_2{\rbrace}$, and
$L_1\cap L_2={\lbrace}w~|~w\in L_1\mbox{ and } w\in L_2{\rbrace}$.

A finite-word automaton is a tuple $A=(Q,\Sigma,q_0,\delta,F)$, where
$Q$ is a finite set of {\em states\/}, $\Sigma$ is a finite alphabet,
$q_0 \in Q$ is an {\em initial state\/}, $\delta: Q\times \Sigma
\rightarrow 2^Q$ is a {\em transition function\/} ($ \delta: Q\times
\Sigma \rightarrow Q$ if the automaton is deterministic), and $F
\subseteq Q$ is a set of {\em accepting\/} states. A triple $(s,a,s')$
such that $s' \in \delta(s,a)$ ($s' = \delta(s,a)$ if the automaton is
deterministic) is a {\em transition labeled by} $a$. A {\em run\/}
$\pi$ of $A$ on a word $w$ is a {\em finite} sequence of states
$s_0s_1s_2{\dots}s_n$ such that for all $1~{\geq}i{\geq}~n$ : $s_{i}
\in \delta(s_{i-1}, w(i))$ (or $s_{i} = \delta(s_{i-1}, w(i))$). The
run $\pi$ is {\em accepting\/} if $s_n \in F$. A word $w$ is accepted
by a finite-word automaton iff that automaton admits at least one
accepting run on $w$. The set of words accepted by $A$ is the {\em
language accepted by $A$}, and is denoted $L(A)$. A language
$L~{\subseteq}~\Sigma^*$ is {\em regular} if it can be accepted by a
finite-state automaton. The language accepted from a state $q$ $\in$
$Q$ is the language accepted by $A$ when considering $q$ to be the
unique initial state. The automaton $A$ is {\em nonempty} if $L(A)
\not= \emptyset$. Deciding if $L(A) \not= \emptyset$ can be done in
linear time. Operations of intersection, union, determinization,
complementation, and minimization of finite-word automata are easily
implementable \cite{Hop71}. Note also that finite-word automata admit
a minimal form which is unique up to isomorphism \cite{Hop71}.

A {\em B\"uchi automaton\/} $A=(Q,\Sigma,q_0,\delta,F)$ is an
automaton that accepts $\omega$-words. A {\em run\/} $\pi$ of $A$ on
an $\omega$-word $w$ is an {\em infinite} sequence of states
$s_0s_1s_2{\dots}$ such that ${\forall}i~{\geq}~1$ : $s_{i} \in
\delta(s_{i-1}, w(i))$ (or $s_{i} = \delta(s_{i-1}, w(i))$.  Let
$\infi (\pi)$ denote the set of states that occur infinitely often in
a run $\pi$. The run $\pi$ {\em accepted\/} if $\infi (\pi) \cap F
\neq \emptyset$. An $\omega$-word $w$ is {\em accepted\/} by a B\"uchi
automaton iff that automaton admits at least one accepting run on
$w$. The language $L(A)$ {\em accepted\/} by a B\"uchi automaton $A$
is the set of $\omega$-words it accepts. The language accepted by a
state $q$ $\in$ $Q$ is defined similarly to the finite-word case. A
language $L \subseteq \Sigma^{\omega}$ is {\em omega-regular\/} if it
can be accepted by a B\"uchi automaton. Deciding if $L(A) \not=
\emptyset$ can be done in linear time. Though the union and
intersection of B\"uchi automata can be computed efficiently
\cite{Buc62}, the complementation operation requires intricate
algorithms that are worst-case exponential
\cite{Buc62,KV01}. Moreover, B\"uchi automata do not admit a unique
minimal form \cite{Buc62}.  

In the rest of this article, we will distinguish between finite-words,
and B\"uchi automata only when this is needed. We conclude the section
by introducing the concept of {\em strongly connected component}.

\begin{definition}
Given an automaton $A=(Q,\Sigma,q_0,\delta,F)$ we define a relation
$\approx$ between its states such that if $q \approx q'$ then either
$q$ $=$ $q'$, or there exists a path from $q$ to $q'$ and a path from
$q'$ to $q$ in the transition graph of $A$. The equivalence classes of
states induced by $\approx$ are {\em the strongly connected
components} of $A$.
\end{definition}

\subsection{Weak B\"uchi Automata}

We now introduce {\em weak\/} automata~\cite{MSS86}. For a B\"uchi
automaton $A=(Q,\Sigma,q_0,\delta,F)$ to be weak, there has to be
partition of its state set $Q$ into disjoint subsets $Q_1, \ldots,
Q_m$ such that for each of the $Q_i$, either $Q_i \subseteq F$, or
$Q_i \cap F = \emptyset$, and there is a partial order $\leq$ on the
sets $Q_1, \ldots, Q_m$ such that for every $q \in Q_i$ and $q'\in
Q_j$ for which, for some $a \in \Sigma$, $q'\in \delta(q,a)$
($q'=\delta(q,a)$ in the deterministic case), $Q_j \leq Q_i$. A weak
automaton is thus a B\"uchi automaton such that each of the strongly
connected components of its graph contains either only accepting or
only non-accepting states, and transitions leaving a component always
move to a lower one.

Not all omega-regular languages can be accepted by weak deterministic
B\"uchi automata, nor even by weak nondeterministic automata. However,
there are algorithmic advantages to working with weak automata: Weak
deterministic automata can be complemented simply by inverting their
accepting and non-accepting states; and there exists a simple
determinization procedure for weak automata~\cite{Saf92}, which
produces B\"uchi automata that are deterministic, but generally not
weak.

Nevertheless, if the represented language can be accepted by a weak
deterministic automaton, the result of the determinization procedure
will be {\em inherently weak\/} according to the definition
below~\cite{BJW01} and thus easily transformed into a weak automaton.

\begin{definition}
A B\"uchi automaton is {\em inherently weak\/} if none of the
reachable strongly connected components of its transition graph
contain both accepting (visiting at least one accepting state) and
non-accepting (not visiting any accepting state) cycles.
\end{definition}

Checking whether a B\"uchi automaton is inherently weak is equivalent
to check if there exists a path in an accepting strongly connected
component of the graph induced by the B\"uchi automaton that do not
pass by an accepting state. This problem can be solved by removing all
accepting states belonging to the strongly connected component, and
then check if there is still a cycle in the resulting graph. Finally,
a major advantage of weak deterministic B\"uchi automata is that they
admit a normal form, which is unique up to isomorphism \cite{Loe01}.If
the strongly connected component contains both accepting and non
accepting states, the problem can be solved by removing all accepting
states, and then check if there still exists a cycle in the resulting
graph.

                                      
\subsection{Binary Relations and Transducers}
\label{transdu}

A finite-word (resp infinite-word) {\em relation\/} $R$ over a finite
alphabet $\Sigma{\times}\Sigma$ is a set of pairs of finite
(resp. infinite) words over $\Sigma$. The {\em identity relation}
$R_{id}$ is the set of all pairs $(w,w')$ such that $w=w'$. The
relation $R$ is {\em reflexive} iff $R_{id}~{\subseteq}~R$. Given two
relations $R_1$ and $R_2$, their composition $R_{12}=R_1{\circ}R_2$ is
a relation such that for each pair $(w,w')$ $\in$ $R_1 {\circ} R_2$,
there exists $w''$ with $(w,w'')$ $\in$ $R_1$ and $(w'',w')$ $\in$
$R_2$. The image of a set of words $\phi_1$ by $R$ is the set of words
$\phi_2$ such that for each $w'$ $\in$ $\phi_2$, there exists $w$
$\in$ $\phi_1$ with $(w,w')$ $\in$ $R$.  We denote by $R^i$ the
relation obtained by composing $i$ times $R$ with itself. The
reflexive transitive closure of $R$ is
$R^*=\bigcup_{i=0}^{\infty}R^i$; its transitive closure $R^+$ is
$R^+=R{\circ}R^*$.

Several classes of relations can be represented by {\em
transducers}. In this article, a finite-word (resp. B\"uchi (weak))
transducer $T=(Q, {\Sigma}{\times}{\Sigma}, q_{0}, \delta, F)$ is an
automaton operating on {\em pairs} of symbols rather than on a {\em
single} symbol. A relation $R$ is representable by $T$ iff $R =
L(T)$. Depending of their accepting condition, transducers can define
various types of relations. A finite-word relation that is represented
by a finite-word transducer is called a {\em length-preserving regular
relation}, and an infinite-word relation which is represented by a
B\"uchi (weak) transducer is called an {\em omega (weak) relation}.

Operations between relations can be defined on their corresponding
transducers. In the rest of this section, we consider
length-preserving regular relations, and omega weak
relations.

Let $T_1=(Q_1, {\Sigma}{\times}{\Sigma}, q_{01}, \delta_1, F_1)$ and
$T_2=(Q_2, {\Sigma}{\times}{\Sigma}, q_{02}, \delta_2, F_2)$ be two
transducers representing respectively $R_1$ and $R_2$, and $A = (Q ,
\Sigma, q_{0},\delta ,F )$ an automaton for the set $\phi_1$.

The relation $R_{12}= R_1 {\circ} R_2$ is represented by the
finite-word (resp. B\"uchi weak) transducer $T_{12} =(Q_1{\times}Q_2,
\Sigma{\times}\Sigma,$ $ (q_{01},q_{02}), \delta_{12},
F_1{\times}F_2)$, where
\[\delta_{12}((q_1,q_2),(a,b))=\{(q'_1,q'_2)\mid (\exists c \in \Sigma) 
(q'_1 \in \delta_1(q_1,(a,c))\ \mbox{and}\ q'_2 \in
\delta_2(q_2,(c,b)))\}.\]

The set $R_1(\phi)$ is represented by the finite-word (resp. B\"uchi
weak) automaton $T_1(A )=(Q_1{\times}Q , \Sigma, (q_{01},q_{03}),
\delta_{13}, F_1{\times}F )$, where
\[\delta_{13}((q_1,q ),b)=\{(q'_1,q' )\mid (q'_1 \in \delta_1(q_1,(a,b))\ \mbox{and}\ q'  \in
\delta (q ,a))\}.\]

It is easy to see that $R_1^*(\phi)$ is representable by
$\bigcup_{i}T^{i}(A)$, and $R^*$ by $\bigcup_{i}T$.

Note that the composition of two B\"uchi weak automata is a
non-deterministic B\"uchi weak automaton. However, there are no
guaranties that this property will be preserved after determinization.
This can be checked using the technique presented at the end of
Section \ref{automata-intro}.

\input{counters}


==> figs/preliminaries.tex <==
\section{Preliminaries}

In this section, we introduce the theoretical concepts that will be
used in the rest of this article.

\subsection{Languages and Automata}
\label{automata-intro}

A {\em finite word\/} $w$ over a finite alphabet $\Sigma$ is a finite
sequence of elements of $\Sigma$. An {\em infinite word \/}(or {\em
$\omega$-word\/}) $w$ over $\Sigma$ is a countably infinite sequence
of elements of $\Sigma$. The $i-th$ element (also called symbol) of
the sequence $w$ is denoted by $w(i)$.  The set of finite and infinite
words over $\Sigma$ are respectively denoted by $\Sigma^*$ and
$\Sigma^{\omega}$. A language on $\Sigma$ is a set of words over
$\Sigma$. The complement of $L$ is defined by
$\bar{L}={\lbrace}w|w\notin L{\rbrace}$. Given two languages $L_1$
and $L_2$, their union and intersection are respectively defined by
$L_1\cup L_2={\lbrace}w|w\in L_1\mbox{ or } w\in L_2{\rbrace}$, and
$L_1\cap L_2={\lbrace}w|w\in L_1\mbox{ and } w\in L_2{\rbrace}$.

A finite-word automaton is a tuple $A=(Q,\Sigma,q_0,\delta,F)$, where
$Q$ is a finite set of {\em states\/}, $\Sigma$ is a finite alphabet,
$q_0 \in Q$ is an {\em initial state\/}, $\delta: Q\times \Sigma
\rightarrow 2^Q$ is a {\em transition function\/} ($ \delta: Q\times
\Sigma \rightarrow Q$ if the automaton is deterministic), and $F
\subseteq Q$ is a set of {\em accepting\/} states. A triple $(s,a,s')$
such that $s' \in \delta(s,a)$ (or $s' = \delta(s,a)$ if the automaton
is deterministic) is a {\em transition labeled by} $a$. A {\em run\/}
$\pi$ of $A$ on a finite word $w$ is a {\em finite} sequence of states
$s_0s_1s_2{\dots}s_n$ such that for all $1~{\leq}i{\leq}~n$ : $s_{i}
\in \delta(s_{i-1}, w(i))$ (or $s_{i} = \delta(s_{i-1}, w(i))$). The
run $\pi$ is {\em accepting\/} if $s_n \in F$. A {\em B\"uchi
automaton\/} $A=(Q,\Sigma,q_0,\delta,F)$ is an automaton that accepts
$\omega$-words; its syntax is equivalent to the one of a finite-word
automaton. A {\em run\/} $\pi$ of $A$ on an $\omega$-word $w$ is an
{\em infinite} sequence of states $s_0s_1s_2{\dots}$ such that
${\forall}i~{\geq}~1$ : $s_{i} \in \delta(s_{i-1}, w(i))$ (or $s_{i} =
\delta(s_{i-1}, w(i))$.  Let $\infi (\pi)$ denote the set of states
that occur infinitely often in a run $\pi$. The run $\pi$ {\em
accepted\/} if $\infi (\pi) \cap F \neq \emptyset$. In the rest of
this article, we will distinguish between finite-words, and B\"uchi
automata only when this is needed.

Given an automaton $A=(Q,\Sigma,q_0,\delta,F)$, a word $w$ is accepted
by $A$ iff that automaton admits at least one accepting run on
$w$. The set of words accepted by $A$ is the {\em language accepted by
$A$}, and is denoted $L(A)$. A language $L$ is {\em regular} if it can
be accepted by a finite-state automaton; it is {\em
$\omega$-regular\/} if it can be accepted by a B\"uchi automaton.  The
language accepted from a state $q$ $\in$ $Q$ is the language accepted
by $A$ when considering $q$ to be the unique initial state. The
automaton $A$ is {\em nonempty} if $L(A) \not= \emptyset$. Deciding if
$L(A) \not= \emptyset$ can be done in linear time in both cases
\cite{Buc62,Hop71}. We can define a relation $\approx$ between the
states of $A$ such that if $q \approx q'$ then either $q$ $=$ $q'$, or
there exists a path from $q$ to $q'$ and a path from $q'$ to $q$ in
the transition graph of $A$. The equivalence classes of states induced
by $\approx$ are {\em the strongly connected components} of $A$.

Both finite-word and B\"uchi automata are closed under intersection
and union. However, while finite-word automata are closed under
determinization, there exist B\"uchi automata that do not admit a
deterministic form \cite{Buc62}. Complementation for finite-word
automata involves an exponential blow up with a linear exponent, which
is due to the necessity of applying a determinization before
performing the operation. Complementation for B\"uchi automata is also
exponential \cite{Buc62,KV01,KV04}, but in this case, the exponent is
nonlinear, while it is only linear in the finite-word case. This
explain why complementation for B\"uchi automata is harder than
complementation for finite-word automata (see \cite{Var95,KV04} for a
discussion). Finally, it is worth mentioning that, oppositely to
B\"uchi automata, finite-word automata admit a minimal form which is
unique up to isomorphism \cite{Buc62,Hop71}.

\subsection{B\"uchi Weak Automata}

We now introduce {\em weak\/} automata~\cite{MSS86}. For a B\"uchi
automaton $A=(Q,\Sigma,q_0,\delta,F)$ to be weak, there has to be
partition of its state set $Q$ into disjoint subsets $Q_1, \ldots,
Q_m$ such that for each of the $Q_i$, either $Q_i \subseteq F$, or
$Q_i \cap F = \emptyset$, and there is a partial order $\leq$ on the
sets $Q_1, \ldots, Q_m$ such that for every $q \in Q_i$ and $q'\in
Q_j$ for which, for some $a \in \Sigma$, $q'\in \delta(q,a)$
($q'=\delta(q,a)$ in the deterministic case), $Q_j \leq Q_i$. A weak
automaton is thus a B\"uchi automaton such that each of the strongly
connected components of its graph contains either only accepting or
only non-accepting states, and transitions leaving a component always
move to a lower one.

Not all $\omega$-regular languages can be accepted by weak deterministic
B\"uchi automata, nor even by weak nondeterministic automata. However,
there are algorithmic advantages to working with weak automata: Weak
deterministic automata can be complemented simply by inverting their
accepting and non-accepting states; and there exists a simple
determinization procedure for weak automata~\cite{Saf92}, which
produces B\"uchi automata that are deterministic, but generally not
weak.

Nevertheless, if the represented language can be accepted by a weak
deterministic automaton, the result of the determinization procedure
will be {\em inherently weak\/} according to the definition
below~\cite{BJW01} and thus easily transformed into a weak automaton.

\begin{definition}
A B\"uchi automaton is {\em inherently weak\/} if none of the
reachable strongly connected components of its transition graph
contain both accepting (visiting at least one accepting state) and
non-accepting (not visiting any accepting state) cycles.
\end{definition}

Checking whether a B\"uchi automaton is inherently weak is equivalent
to check if there exists a path in an accepting strongly connected
component of the graph induced by the B\"uchi automaton that do not
pass by an accepting state. This problem can be solved by removing all
accepting states belonging to the strongly connected component, and
then check if there is still a cycle in the resulting graph. Finally,
a major advantage of weak deterministic B\"uchi automata is that they
admit a normal form, which is unique up to isomorphism \cite{Loe01}.If
the strongly connected component contains both accepting and non
accepting states, the problem can be solved by removing all accepting
states, and then check if there still exists a cycle in the resulting
graph.

                                      
\subsection{Binary Relations and Transducers}
\label{transdu}

A finite-word (resp $\omega$-word) {\em relation\/} $R$ over a finite
alphabet $\Sigma{\times}\Sigma$ is a set of pairs of finite words
(resp. $\omega$-words) over $\Sigma$. The {\em identity relation}
$R_{id}$ is the set of all pairs $(w,w')$ such that $w=w'$. The
relation $R$ is {\em reflexive} iff $R_{id}~{\subseteq}~R$. Given two
relations $R_1$ and $R_2$, their composition $R_{12}=R_1{\circ}R_2$ is
a relation such that for each pair $(w,w')$ $\in$ $R_1 {\circ} R_2$,
there exists $w''$ with $(w,w'')$ $\in$ $R_1$ and $(w'',w')$ $\in$
$R_2$. The image of a set of words $\phi_1$ by $R$ is the set of words
$\phi_2$ such that for each $w'$ $\in$ $\phi_2$, there exists $w$
$\in$ $\phi_1$ with $(w,w')$ $\in$ $R$.  We denote by $R^i$ the
relation obtained by composing $i$ times $R$ with itself. The
reflexive transitive closure of $R$ is
$R^*=\bigcup_{i=0}^{\infty}R^i$; its transitive closure $R^+$ is
$R^+=R{\circ}R^*$.

Several classes of relations can be represented by {\em
transducers}. In this article, a finite-word (resp. B\"uchi (weak))
transducer $T=(Q, {\Sigma}{\times}{\Sigma}, q_{0}, \delta, F)$ is an
automaton operating on {\em pairs} of symbols rather than on a {\em
single} symbol. A relation $R$ is representable by $T$ iff $R =
L(T)$. Depending of their accepting condition, transducers can define
various types of relations. A finite-word relation that is represented
by a finite-word transducer is called a {\em length-preserving regular
relation}, and an $\omega$-word relation which is represented by a
B\"uchi (weak) transducer is called an {\em omega (weak) relation}.

Operations between relations can be defined on their corresponding
transducers. In the rest of this section, we consider
length-preserving regular relations, and omega weak
relations.

Let $T_1=(Q_1, {\Sigma}{\times}{\Sigma}, q_{01}, \delta_1, F_1)$ and
$T_2=(Q_2, {\Sigma}{\times}{\Sigma}, q_{02}, \delta_2, F_2)$ be two
transducers representing respectively $R_1$ and $R_2$, and $A = (Q ,
\Sigma, q_{0},\delta ,F )$ an automaton for the set $\phi_1$.

The relation $R_{12}= R_1 {\circ} R_2$ is represented by the
finite-word (resp. B\"uchi weak) transducer $T_{12} =(Q_1{\times}Q_2,
\Sigma{\times}\Sigma,$ $ (q_{01},q_{02}), \delta_{12},
F_1{\times}F_2)$, where
\[\delta_{12}((q_1,q_2),(a,b))=\{(q'_1,q'_2)\mid (\exists c \in \Sigma) 
(q'_1 \in \delta_1(q_1,(a,c))\ \mbox{and}\ q'_2 \in
\delta_2(q_2,(c,b)))\}.\]

The set $R_1(\phi)$ is represented by the finite-word (resp. B\"uchi
weak) automaton $T_1(A )=(Q_1{\times}Q , \Sigma, (q_{01},q_{03}),
\delta_{13}, F_1{\times}F )$, where
\[\delta_{13}((q_1,q ),b)=\{(q'_1,q' )\mid (q'_1 \in \delta_1(q_1,(a,b))\ \mbox{and}\ q'  \in
\delta (q ,a))\}.\]

It is easy to see that $R_1^*(\phi)$ is representable by
$\bigcup_{i}T^{i}(A)$, and $R^*$ by $\bigcup_{i}T$.

Note that the composition of two B\"uchi weak automata is a
non-deterministic B\"uchi weak automaton. However, there are no
guaranties that this property will be preserved after determinization.
This can be checked using the technique presented at the end of
Section \ref{automata-intro}.

\input{counters}


==> figs/weak-extra.tex <==
\subsection{The $\omega$-Word Case}
\label{weak1}

In this section, we generalize the results of Section \ref{extra} to
deterministic B\"uchi weak automata. Our first idea was to use
Algorithm \ref{closure_algo_1}. However the following example shows
that this algorithm fails when considering $\omega$-words.

\begin{example}
\label{failure-closure}
Consider the B\"uchi weak automata $A^{1}$, $A^{2}$ and $A^{3}$
depicted in Figure \ref{example-auto}, and first do not consider the
dashed transition in $A_{3}$. Those three automata form an
incrementally growing sequence if the dashed transition is not
considered. The increment detected between $A^{1}$ and $A^{2}$ is
denoted by $Q_{I_O}^{2}$ and the one between $A^{2}$ and $A^{3}$ by
$Q_{I_0}^{3}$. The application of Algorithm \ref{closure_algo_1} to
$A^{3}$ will add the dashed transition. The language of the
extrapolated automaton will accept words of the form
$a^{*}c^{\omega}$. Those words cannot be accepted by an automaton
obtained by adding a finite number of increments to $A^{3}$.
\end{example}

\begin{figure}
\begin{center}
\input{figs/example.pstex_t}
\end{center}
\caption{Failure of Algorithm \ref{closure_algo_2} for the $\omega$-words case.}
\label{example-auto}
\end{figure}

Each word $w\in L(A^{e_{i>0}})$ is the concatenation of a finite
prefix with an infinite suffix that is generated by a strongly
connected component of $A^{e_i}$. Since the increments added between
$A^{e_0}$ and $A^{e_i}$ are isomorphic to $Q_{I_0}^{e_0}$, each
strongly connected component $sc$ $\in$ $Q^{e_i}\cup Q^{e_*}$ must be
isomorphic to a strongly connected component in $A^{e_0}$. As it has
been illustrated in Example \ref{failure-closure}, this is not always
the case when applying Algorithm \ref{closure_algo_1}.

A solution to this problem is to ensure that the transitions added
during the extrapolation process will not introduce new accepting
strongly connected components, i.e. that the intersection between the
new strongly connected components and the set of accepting states of
$A^{e_*}$ will be empty. We get the following algorithm.

\begin{algo}
\label{closure_algo_3}
Consider the deterministic B\"uchi weak automaton $A^{i+k} = A^{e_0} =
(Q^{e_0}, \Sigma, q_0^{e_0}, \delta^{e_0}, F^{e_0})$. We build a
B\"uchi weak automaton ${A^{e_*}} = (Q^{e_*}, \Sigma,$\\$
q_0^{e_*}, \delta^{e_*}, F^{e_*})$, where $Q^{e_*} = Q^{e_0} \cup
Q_{I_{0}COPY}$, $q_0^{e_*} = q_0^{e_0}$,
$|Q_{I_{0}COPY}|=|Q_{I_0}^{e_0}|$ , and $F^{e_*} = F^{e_0}$. Each
state $q^{e_0}$ of $A^{e_0}$ is associated to exactly one state
$q^{e_*}$ of ${A^{e_*}}$ by a relation
$\equiv_1~{\subseteq}~Q^{e_0} \times
(Q^{e_*}-Q_{I_{0}COPY}^{e_*})$. Moreover $Q^{e_*}-Q_{I_{0}COPY}$ can
be decomposed into $Q_H^{e_0}~{\equiv_1}~Q_H^{e_*}$, a series of $k$
increments $Q_{I_0}^{e_0}~{\equiv_1}~Q_{I_0}^{e_*}, \ldots,
Q_{I_{k-1}}^{e_0}~{\equiv_1}~Q_{I_{k-1}}^{e_*}$, and a final tail
$Q_{T_f}^{e_0}~{\equiv_1}~Q_{T_f}^{e_*}$.  The set $Q_{I_{0}COPY}$ is
used to create a copy of $Q_{I_{0}}^{e_0}$.  Each state of
$Q_{I_{0}COPY}$ is associated to a corresponding state in
$Q_{I_{0}}^{e_*}$ by a relation $\equiv_2~
{\subseteq}~Q_{I_{0}}^{e_*}{\times}Q_{I_{0}COPY}$. The set of
transition is built in the following way. For each transition
$(q_x^{e_0},a,q_y^{e_0})$ in $A^{e_0}$, there exists a transition
$(q_x^{e_*},a,q_y^{e_*})$ in $A^{e_*}$ with $q_x^{e_0} \equiv
q_x^{e_*}$ and $q_y^{e_0}\equiv q_y^{e_*}$.  For each transition
$(q_x^{I_0},a,q_y^{I_0})$ in $A^{e_*}$ with $q_x^{I_0},q_y^{I_0}$
$\in$ $Q_{I_0}^{e_*}$ there exists a transition
$(q_x^{I_{0}COPY},a,q_y^{I_{0}COPY})$ where $q_x^{I_{0}COPY}$ and
$q_y^{I_{0}COPY}$ $\in$ $Q_{I_{0}COPY}$ and $q_x^{I_0} \equiv_2
q_x^{I_{0}COPY}$ and $q_y^{I_0} \equiv_2 q_y^{I_{0}COPY}$.  For each
transition $(q_x^{I_0},a,q_y^{e_*})$ in $A^{e_*}$ with $q_x^{I_0}$
$\in$ $Q_{I_0}^{e_*}$ and $q_y^{e_*}$ $\not\in$ $Q_{I_0}^{e_*}$, there
exists a transition $(q_x^{I_{0}COPY},a,q_y^{e_*})$ where
$q_x^{I_{0}COPY}$ $\in$ $Q_{I_{0}COPY}$ and $q_x^{e_*}
\equiv_2q_x^{I_{0}COPY} $. For each state $q \in Q_{H}^{e_0} \ {\cup}
\ Q_{I_0}^{e_0}$ and for every $a \in \Sigma$,
\begin{enumerate}
\item
if $\delta_{e_0}(q_x^{e_0},a)$ is a state $q_y^{e_0}$ that belong to
an increment $Q_{I_{j}}^{e_0}$, $1\leq j \leq k -1$, then for each
increment $Q_{I_{\ell}}^{e_*}$ with $0 < \ell < j$, there is a
transition $(q_x^{e_*},a,(q_y^{e_*})')$ in ${A^{e_*}}$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$, with $q_x^{e_0}
\equiv_1 q_x^{e_*}$ and $q_y^{e_0} \equiv_1 q_y^{e_*}$. There is also
a transition $(q_x^{e_*},a,q_y^{I_{0}COPY})$, where
$q_y^{I_{0}COPY}$ is the state corresponding to $q_y^{e_*}$ in
$Q_{I_{0}COPY}$ by the increment isomorphism.
\item
if $q$ $\in$ $Q^{e_0}_{I_0}$ then let $q^{I_{0}COPY}$ be the state
corresponding to $q$ in $Q_{I_{0}COPY}$ (i.e. $(q,q^{I_{O}COPY}$) $\in$
$\equiv_2 {\circ} \equiv_1$ ). For each increment $Q_{I_{\ell}}^{e_*}$
with $1~{\leq}~l < j$, there is a transition
$(q^{I_{0}COPY},a,(q_y^{e_*})')$ in ${A^{e_*}}$ , where
$(q_y^{e_*})'$ is the state corresponding to $q_y^{e_*}$ (by the
increment isomorphism) in $Q_{I_{\ell}}^{e_*}$ There is also a
transition $(q_{I_{0}COPY},a,q_y^{I_{0}COPY})$, where
$q_y^{I_{0}COPY}$ is the state corresponding to $q_y^{e_*}$ in\\
$Q_{I_{0}COPY}$.
\end{enumerate}
\end{algo}

These construction rules allow to simulate the computations of any of
the $Q^{e_i}$, $i\geq 0$. Notice that the transitions added at the
last step may introduce new cycles from states of $Q_{I_{0}COPY}$ to
themselves (following these cycles amounts to visiting some additional
number of increments). Since the accepting runs of the $A^{e_i}$ can
only go through a finite number of increments, it is essential to make
these cycles non-accepting, which is the reason behind the duplication
of the first increment into $Q_{I_{0}COPY}$.

\begin{figure}
\begin{center}
\input{figs/example3.pstex_t}
\end{center}
\caption{Application of Algorithm \ref{closure_algo_3} to the automaton
of Figure \ref{example-auto}}.
\label{example-auto21}
\end{figure}

\begin{example}
Figure \ref{example-auto21} shows the result of applying Algorithm
\ref{closure_algo_3} to the automaton $A^{3}$ of Figure
\ref{example-auto}.
\end{example}

A formal proof of correctness of algorithm
\ref{closure_algo_3} will be given in Section
\ref{count}.

\input{extra-count}

==> figs/weak-precis.tex <==
\section{Safety and Preciseness for B\"uchi Weak Automata}
\label{weak2}

In this section, we generalize the results of Section
\ref{safe-precis} to B\"uchi weak deterministic automata.
We provide sufficient criteria to ensure that the
extrapolation of a sequence of B\"uchi weak deterministic automata is
safe and precise. Like in Section \ref{safe-precis} we provide
criteria for both problems presented in Section \ref{model}.

\subsection{Transitive Closure of a Relation}

In this section, we consider $T^{e_*}$ to be transducer obtained by
applying algorithm \ref{closure_algo_3} to the last transducer
$T^{i+k}$ of an incrementally growing sampling sequence $T^{i}, T^{i +
1}, \dots, T^{i+k-1}, T^{i+k}$ of powers of a reflexive transducer
$T$. By construction $L_{\omega}(T^{e_*}) =
L_{\omega}(\cup_iT^{e_i})$, where $T^{e_0} = T^{i+k}$ and $\forall i >
0$ $T^{e_i}$ is the automaton obtained from $T^{e_0}$ by adding $i$
increments communication equivalent to the increment detected between
$T^{i+k-1}$ and $T^{i+k}$ by applying Algorithm \ref{closure_algo_3}.

We now propose a sufficient condition for checking the safetiness of
our extrapolation. The condition is presented under the form of a
theorem.

\begin{theorem}
\label{safe2}
The transducer $T^{e_*}$ is a safe extrapolation of $T$ if\\
$L_{\omega}(T^{e_*} \circ T^{e_*}) \subseteq L_{\omega}(T^{e_*})$.
\end{theorem}

\begin{proof}
Same as the one of Theorem \ref{safe1}.
\end{proof}

In practice, checking the condition expressed by Lemma \ref{safe2}
requires to complement $T_0^{e_*}$.  By construction, this transducer
is weak but generally not deterministic. The solution we implemented
consists in determinizing $T_0^{e_*}$, and then checking whether the
resulting transducer is inherently weak. In the positive case, this
transducer can be turned into a weak deterministic one and easily
complemented. Otherwise, the test cannot be completed.  An another
solution could be to implement one of the complementation
constructions presented in \cite{KV01,CKV03,KV04,FKV04}.

We now examinate the problem of providing a sufficient criterion for
ensuring preciseness of our construction.

Following a same argument as the one provided in Section
\ref{subsec-transd} we have that $T^{e_*}$ is precise if

\begin{equation}
\label{extra-weak}
 \forall w \in (\Sigma {\times} \Sigma)^*, {\forall} i >0 \
{\lbrack}w \in L_{\omega}(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w \in
L_{\omega}(T^{e_j}{\circ}T^{e_j'}){\rbrack}.
\end{equation}

Which can be reduce to the following condition by using counter automata.


%% the following proof is very similar to the case of finite words!.

\begin{equation}
\label{equa-precis1}
L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c (T_{c_2}^{e_*}
\circ_c T_{c_3}^{e_{*}}){\rbrack})= L_{\omega}(T_{c_1}^{e_*}).
\end{equation}

We have the following theorem.

\begin{theorem}
We have that $L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*}
\cap_c (T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})=
L_{\omega}(T_{c_1}^{e_*})$ is satisfied iff $\forall w \in (\Sigma
{\times} \Sigma)^*, {\forall} i >0 \ {\lbrack}w \in
L_{\omega}(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w \in
L_{\omega}(T^{e_j}{\circ}T^{e_j'}){\rbrack}$ is satisfied.
\end{theorem}

\begin{proof}
We prove the two senses of the equivalence.
\begin{enumerate}
\item
We show that if $ L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c
(T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})= L_{\omega}(T_{c_1}^{e_*})$,
then $\forall w \in (\Sigma {\times} \Sigma)^*, {\forall} i >0 \
{\lbrack}w \in L_{\omega}(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w \in
L_{\omega}(T^{e_j}{\circ}T^{e_j'}){\rbrack}$. For each $w$ $\in$ $(\Sigma
{\times} {\Sigma})^{*}$, if $w$ $\in$ $T^{e_i}$ and $w$ $\not\in$
$T^{e_{j<i}}$ then, by Theorem \ref{th-algo-count2}, there exists
$w_c$ $\in$ $L_{\omega}(T_{c_1}^{e_*})$ such that $P(w_c) = (w,i)$. Since
Condition \ref{equa-precis1} holds, there exists $w_c'$, $w_c''$ $\in$
$T^{e_*}_{c_1}$ such that $P(w_c') = (w',j)$ and $P(w_c'') = (w'',j')$
with $j,j'<i$ and $w = w'{\circ} w''$. By theorem
\ref{th-algo-count2}, $w'$ $\in$ $T^{e_j}$ and $w''$ $\in$
$L_{\omega}(T^{e_{j'}})$.
\item
We show that if $\forall w \in (\Sigma {\times} \Sigma)^*, {\forall} i
>0 \ {\lbrack}w \in L_{\omega}(T^{e_i}) \ {\Rightarrow} \ {\exists}j,j'<i, w
\in L_{\omega}(T^{e_j}{\circ}T^{e_j'}){\rbrack}$, then
$L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c (T_{c_2}^{e_*}
\circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*})$. We must show
that each word $w_c$ $\in$ $L_{\omega}(A^{e_*}_{c_1})$ with $P(w_c)=(w,i>0)$
can be obtained from two words $w_c'$ and $w_c''$ $\in$
$T^{e_*}_{c_1}$, where $P(w_c')=(w',l<i)$, $P(w_c'')=(w'',l'<i)$, and
$w = w' {\circ} w''$. By theorem \ref{th-algo-count2}, $w$ $\in$
$T^{e_i}$. Since Condition \ref{extra1} is satisfied, there exists
$w'$ $\in$ $T^{e_{j<i}}$ and $w''$ $\in$ $T^{e_{j'<i}}$ with $w = w'
{\circ} w''$. By theorem \ref{th-algo-count2}, there exists also
$w_c'$, $w_c''$ $\in$ $L_{\omega}(A^{e_*}_c)$ with $P(w_c')=(w',l {\leq} j)$
and $P(w_c'')=(w'',l' {\leq} j')$.
\end{enumerate}
\end{proof}

The computation of
$L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*} \cap_c
(T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})= L(T_{c_1}^{e_*})$
can be done by using a principe similar to the one described in
Section \ref{subsec-transd}.

Notice that in practice checking Condition \ref{} requires to
complement $L_{\omega}({\pi}_{c_1>c_2,c_3}{\lbrack}T_{c_1}^{e_*}
\cap_c (T_{c_2}^{e_*} \circ_c T_{c_3}^{e_{*}}){\rbrack})$. To this
purpose, we follow the same principle as the one given for checking
\lemma, i.e.

\label{Limit of a Sequence of Reachable Sets}

==> heuristics.tex <==
\section{Implementation Issues}

%% list all of them.


